New Direct Sum Tests

A function $f:[n]^{d} \to \mathbb{F}_2$ is a \defn{direct sum} if there are functions $L_i:[n]\to \mathbb{F}_2$ such that ${f(x) = \sum_{i}L_i(x_i)}$. In this work we give multiple results related to the property testing of direct sums. Our first result concerns a test proposed by Dinur and Golubev in 2019. We call their test the Diamond test and show that it is indeed a direct sum tester. More specifically, we show that if a function $f$ is $\epsilon$-far from being a direct sum function, then the Diamond test rejects $f$ with probability at least $\Omega_{n,\epsilon}(1)$. Even in the case of $n = 2$, the Diamond test is, to the best of our knowledge, novel and yields a new tester for the classic property of affinity. Apart from the Diamond test, we also analyze a broad family of direct sum tests, which at a high level, run an arbitrary affinity test on the restriction of $f$ to a random hypercube inside of $[n]^d$. This family of tests includes the direct sum test analyzed in \cite{di19}, but does not include the Diamond test. As an application of our result, we obtain a direct sum test which works in the online adversary model of \cite{KRV}. Finally, we also discuss a Fourier analytic interpretation of the diamond tester in the $n=2$ case, as well as prove local correction results for direct sum as conjectured by Dinur and Golubev.

==> applications.tex <==
\section{Applications}

In this section we state some corollaries that follow as applications of our results in \cref{sec:diamond}. 

\input{fourierfact}

==> diamond-4.tex <==
\newcommand{\DP}{\mathcal{D}_p}
\section{The Diamond Test}\label{sec:diamond}
We restate the Diamond in the Cube test, initially proposed by Dinur and Golubev in \cite{di19} (recall from \cref{sec:prelims} that $\phi_x$ is the interpolation function)
\begin{test}[Diamond in Cube]\label{test:diamondcube}
Sample random $a,b\in [n]^d,x\in \F_2^d$. Accept iff
$$f(a)+f(b)=f(\phi_x(a,b))+f(\phi_x(b,a)).$$
\end{test}
% We note that, to the best of the authors' knowledge, this test was not
% previously understood in the setting $n=2$. That is, an analysis of the Diamond
% in Cube test for the case $n=2$ gives a novel affinity tester for functions
% $f:\F_2^d\to \F_2$. This is in contrast to Dinur and Golubev's Square in Cube
% test for direct sum, which reduces to the BLR \cite{BLR} tester in the case of
% $n=2$.
We will show that \cref{test:diamondcube} is a valid tester for direct sum. As is usual in property testing, 
it is straightforward to verify that any direct sum passes with probability $1$ and so completeness holds. The remainder of the section is focused on showing soundness via the following theorem.

\begin{theorem} \label{thm:diamond_cube_soundness}
    Suppose $f: [n]^d \xrightarrow[]{} \F_2$ passes the Diamond in the Cube Test with probability $1-\epsilon$. Then, $f$ is ... close to a direct sum.
\end{theorem}

Our proof proceeds as follows. We begin by considering a $p$-biased version of the Diamond in the Cube test in the $n = 2$, or hypercube, case --- which we simply call the Diamond test. After establishing soundness in this setting, we then boost to the general $n$ setting by viewing the overall Diamond in the Cube test as choosing a random, induced, hypercube in $[n]^d$, and then performing the $p$-biased Diamond test inside of this hypercube for an appropriately chosen $p$. Altogether, this will give us many local direct sums that nearly agree with $f$ on many induced hypercubes inside of $[n]^d$. To conclude we use a direct product testing result of \cite{dinur2014direct} to show that there is a global direct sum consistent with many of the local direct sums. This global direct sum is also close to $f$ and so we are done. 

The $p$-biased hypercube case is analyzed in \cref{sec: n=2 case}, the application of direct product testing is done in \cref{sec:subcube}, and we conclude the proof of soundness by combining the two parts in \cref{sec:conclude soundness diamond}.

\subsection{Step 1: The $p$-biased $n = 2$ Case} \label{sec: n=2 case}
In this section we consider a $p$-biased version of the Diamond in the Cube Test in the $n = 2$ case. Here it will be convenient for us to view the domain as $\F_2^d$ instead of $[2]^d$ and refer to direct sums over $\F_2^d$ as affine functions. We also refer to \cref{test:diamondcube} simply as the Diamond test for the $n = 2$ case. The $p$-biased generalization of the Diamond test that we consider is the following:
\begin{test}\label{test:diamond test}[$p$-Biased Diamond]
Sample $a,x\sim \F_2^{d}$, and $b\sim \T_p(a)$. Accept if and only if
$$f(a)+f(b)=f(\phi_x(a,b))+f(\phi_x(b,a)).$$
\end{test}
We will often refer to the $p$-Biased Diamond test as simply the Diamond test when $p$ is
clear from context. We encourage the reader to focus on the case of $p=0$ (i.e.,
the Diamond test). We will usually fix $p\in (-1,1)$ before specifying $n,d$,
meaning $|p|$ is thought of as bounded away from $1$ by some constant; the dependence
of our results on this constant will be hidden by our asymptotic notation.

The goal of this section is to show that \cref{test:diamond test} is a valid affinity tester  over $\F_2^d$. As a warm up, let us consider what happens when the test passes with probability $1$. This case will be useful to us later on and also establishes the diamond test's completeness.

\begin{lemma}\label{lem:basecase}
Fix $p\in (-1,1)$. The function
$f: \F_2^d \xrightarrow[]{} \F$ is affine if and only if $f$ passes the $p$-Biased Diamond test with probability $1$.
\end{lemma}
\begin{proof}
If $f$ is affine then we can write $f(x) = \sum_i L_i(x_i)$. It follows that for any $a,b \in \F_2^d$,
$$f(a)+f(b)  = \sum_i (L_i(a_i)+L_i(b_i)) = f(\phi_x(a,b)) + f(\phi_x(b,a)).$$
For the other direction, suppose $f$ passes the Diamond test with probability $1$. Then, for all $x,a\in \F_2^d$ we have
\begin{equation}\label{eq:breakitup}
f(a) = f(0)+f(\phi_x(0,a)) + f(\phi_x(a,0)),
\end{equation}
where $0$ denotes the zero vector. Let $e_i\in \F_2^d$ denote a vector which is
$0$ at all coordinates except coordinate $i$.
Then, repeated application of \cref{eq:breakitup} lets us decompose  $f(a)$ as 
$$f(a) = f(0)+\sum_{i=1}^d \left(f(a_i e_{i})+f(0)\right),$$
indicating that $f$ is affine.
\end{proof}
As a simple corollary of \cref{lem:basecase} we have:
\begin{corollary}
If $f$ is $\eps$-close to affine, then $f$ passes the Diamond test with probability at least $1-4\eps$.
\end{corollary}
\begin{proof}
Let $g$ be affine with $\dist(f,g)\le \eps$. By a union bound, $f$ and $g$ agree
on all $4$  points queried by the test (because each query is marginally
uniformly distributed), in which case the Diamond  test accepts.
by \cref{lem:basecase}.
\end{proof}

With completeness done, the remainder of this section is focused on showing soundness. Specifically, we show the following theorem.
\begin{theorem}\label{cor:1fun}
Fix $p\in (-1,1)$.
If $f$ passes the $p$-Biased Diamond test with probability $1-\eps$, then $f$ is
$O_p(\eps)$-close to affine. 
\end{theorem}

Our analysis of the $n=2$ case is both technically interesting and provides a new result on affinity testing over $\F_2^d$. We start with a rough sketch of the ideas used in the analysis.
First, we will generalize to a ``4-function'' version of the test, which is more amenable to induction.
Then, we use hypercontractivity (\cite{hyper1},\cite{hyper2}) to prove
\cref{thm:dichotomy}, which establishes a dichotomy for 4-tuples of functions
that pass the test with probability $1-\eps$: either the functions are all
$O(\eps)$-close to affine, or one of them is $\Omega(1)$-far from affine.
Next, we will relate the pass probability of $(f,g,h,k)$ to the pass probability of restricted versions $(f,g,h,k)$ with one coordinate fixed. This reduces allows us to go down one dimension and apply induction.
Crucially, the dichotomy theorem allows us to
avoid our closeness factor deteriorating at each step of the induction, which
would result in a dependence on the dimension in our result.
This dichotomy based approach is inspired by the work of \cite{optimalreedmuller, david2015direct}, but
the details of establishing the dichotomy and performing the induction are quite
different.

\subsubsection{The Four Function Version}

In order to facilitate our inductive approach, it will be more convenient to work with a four function version of the diamond test. The one function version of the diamond test can be considered a special case where $f = g= h = k$.
\begin{test}[$p$-Biased 4-Function Diamond]
Sample $a,x\sim \F_2^d, b\sim \T_p(a)$, and accept if and only if
\[ f(a)+k(b) = g(\phi_x(a,b)) + h(\phi_x(b,a)). \] 
\end{test}
The following lemma characterizes what happens when four functions pass with probability $1$. It will be used later to establish the base case (in constant dimensions) of our inductive analysis.
\begin{lemma}\label{lem:4basecase}
Fix $p\in (-1,1)$.
Suppose $(f,g,h,k)$ passes the $p$-Biased 4-function Diamond test with probability $1$.
Then, there is a linear function $L$ such that $f,g,h,k$ are all equal to either $L$ or $L+1$.
\end{lemma}
\begin{proof}
If $(f,g,h,k)$ passes the 4-function Diamond test with probability $1$ then for all $a,x,b$ we have:
\[ f(a)+g(\phi_x(a,b))+h(\phi_x(b,a))+k(b)=0=f(b)+g(\phi_{x+\one}(b,a))+h(\phi_{x+\one}(a,b))+k(a). \] 
Using \cref{fact:fliperoo} to simplify we get that for all $a,b$,
\[ f(a)+k(a)=f(b)+k(b). \] 
Again using the fact that $(f,g,h,k)$ passes the test with probability $1$ we have that for all $a,x,b$:
\[ f(a)+g(\phi_x(a,b))+h(\phi_x(b,a))+k(b)=0=f(a)+g(\phi_{x+\one}(a,b))+h(\phi_{x+\one}(b,a))+k(b). \] 
By \cref{fact:fliperoo} this implies
\[ g(\phi_x(a,b))+g(\phi_{x}(b,a)) = h(\phi_x(a,b))+h(\phi_{x}(b,a)). \] 
Letting $c=\phi_x(a,b),d=\phi_{x}(b,a)$, and noting that $c,d$ can be
arbitrary (unrelated) elements of  $\F_2^{d}$, we have that for all $c,d$.
\[ g(c)+g(d)  = h(c)+h(d).\] 
Combining our observations so far we conclude that there exist constants
$\alpha,\beta$ such that for all $a\in \F_2^{d}$ we have
\[ f(a)=k(a) +\alpha, \quad g(a) = h(a)+\beta.\] 
Thus, for all $a,b$ we have
\[ f(a)+f(b)=g(\phi_x(a,b))+g(\phi_x(b,a))+\alpha+\beta. \] 
Taking $x=0$ we conclude
\[ f(a)+f(b) = g(a)+g(b)+\alpha+\beta. \] 
Thus, there exists $\gamma$ such that  for  all $a$ we have
\[ f(a)=g(a)+\gamma.\] 
In summary, we have shown that for all $a,b,x$, we have
\[ f(a)+f(b)=f(\phi_x(a,b))+f(\phi_x(b,a))+\alpha+\beta. \] 
Setting $x=0$ again shows that $\alpha+\beta = 0$.
Thus, we have that $f$ passes the (1-function) Diamond test with probability $1$.
By \cref{lem:basecase} this implies that $f$ is affine.
Finally, recall that we have shown in the course of our proof that $g,h,k$ all
differ from $f$ by a constant. This concludes the proof.
\end{proof}

\subsubsection{A Dichotomy for Functions Passing the Diamond Test}
We are now prepared to show \cref{thm:dichotomy}, which states
that if the 4-function Diamond test accepts $(f,g,h,k)$ with probability exactly
$1-\eps$ then $f$ is either $O(\eps)$-close to affine, or $\Omega(1)$-far from affine. To this end, we first establish two lemmas which will useful in
the proof. Let $\DP$ denote the following distribution on $(\F_2^{d})^3$:
sample a triple $(a,x,b)$ by first taking $a,x\sim \F_2^{d}$ and then taking
$b\sim\T_p(a)$.

\begin{lemma}\label{lem:fghconst}
Fix $p\in (-1,1)$.
Fix $d\in \N$ and functions $f,g,h:\F_2^{d}\to \F_2$.
Suppose $f,g,h$ have
\[ \Pr_{(a,x,b)\sim\DP}[f(a)+g(\phi_x(a,b))+h(\phi_x(b,a))=1]<\eps. \] 
Then, $f,g,h$ are $3\eps$-close to constants.
\end{lemma}
\begin{proof}
Fix $f,g,h$ as in the theorem. 
Performing a union bound and using \cref{fact:fliperoo} we have
\[ \Pr_{(a,x,b)\sim\DP}[f(a)+g(\phi_x(a,b))+h(\phi_x(b,a))=f(b)+g(\phi_x(a,b))+h(\phi_x(b,a))] >  1-2\eps.\] 
Thus, $f$ is $2\eps$-close to a constant $\alpha$.
Then, by a union bound we have
\[ \Pr_{(a,x,b)\sim\DP}[g(\phi_x(a,b))+h(\phi_x(b,a))=\alpha+1]>1-3\eps. \] 
Of course, the distribution of $(\phi_x(a,b),\phi_x(b,a))$ is the same as the
distribution of $(a,b)$.
Thus, we have
\[ \Pr_{a\sim\F_2^{d},b\sim\T_p(a)}[g(a)+h(b)= \alpha+1]>1-3\eps. \] 
By the probabilistic method this implies that $g,h$ are each $3\eps$-close to
constants.
\end{proof}

We will also need the following lemma, which is a slightly modified version of the classic \defn{small set expansion} property of the noisy hypercube (see \cite{od21}).
\begin{lemma}\label{lem:modifiedhyper}
Fix $p\in (-1, 1)$.
Fix $d\in\N$ and $f,g: \F_2^{d}\to\F_2$. Then,
\[ \Pr_{a\sim\F_2^{d},b\sim \T_p(a)}[f(a) = g(b)=1] \le (\mu(g)\mu(f))^{1/(1+|p|)}. \] 
\end{lemma}
\begin{proof}
We can express the probability in the lemma statement as an inner product:
$\ang{f, g\circ \T_{p}}.$
Using H\"older's inequality and hypercontractivity we have
\begin{align*}
\ang{f, g\circ \T_{p}} \le \norm{f}_{1+|p|}\norm{g\circ \T_{p}}_{1+|p|} \le
\norm{f}_{1+|p|} \norm{g}_{1+|p|} \le (\mu(f)\mu(g))^{1/(1+|p|)}.
\end{align*}
\end{proof}

Now we are ready to establish the dichotomy theorem.
\begin{theorem}\label{thm:dichotomy}
Fix $p\in (-1,1)$. There exists constant $c_p$ such that the following is
true for any $d$ and functions $f,g,h,k:\F_2^{d}\to\F_2$.
Suppose $k$ has $\dist(k, \mathsf{affine})  < c_p$.
Then, the $p$-Biased $4$-function Diamond test rejects $(f,g,h,k)$ with probability at
least $\dist(k,\mathsf{affine})/2$.
\end{theorem}
\begin{proof}
Let $\chi$ be the closest affine function to $k$. Note that
\[ \chi(a)+\chi(b)=\chi(\phi_x(a,b))+\chi(\phi_x(b,a)). \] 
Thus, our goal is equivalent to showing that
\[ \Pr_{(a,x,b)\sim\DP}[(\chi+f)(a)+(\chi+g)(\phi_x(a,b))+(\chi+h)(\phi_x(b,a))\neq
(\chi+k)(b)]\ge \dist(k,\mathsf{affine})/2. \] 
Thus, it suffices to consider the case that the closest affine function to $k$
is the zero function. We assume this for the remainder of the proof. Then,
$\dist(k,\mathsf{affine})=\mu(k)$.
We are already done unless
\begin{equation}
  \label{eq:eatzero}
\Pr_{(a,x,b)\sim\DP}[f(a)+g(\phi_x(a,b))+h(\phi_x(b,a))=1]\le 2\mu(k).
\end{equation}
Thus, we may assume that \cref{eq:eatzero} is true.
Now, by \cref{lem:fghconst} we have that $f,g,h$ are $6\mu(k)$-close to
constants.
Without loss of generality we may assume $g,h$ are both closer to $0$ than to
$1$; otherwise we can add $1$ to both $g,h$, which does not affect the sum
$g(\phi_x(a,b))+h(\phi_x(b,a))$.
If $f$ were closer to $1$ than to $0$ then we would have 
\[ \Pr_{(a,x,b)\sim\DP}[f(a)=1,g(\phi_x(a,b))=h(\phi_x(b,a))=0]\ge 1-18\mu(k) > 2\mu(k), \] 
with the final inequality holding by our assumption that $\mu(k)<c_p$; but this
would contradict \cref{eq:eatzero}, so it cannot happen.
Thus, $f,g,h$ are all $6\mu(k)$-close to $0$.
% Let $$X = \setof{x}{f(x)=1\lor g(x)=1\lor h(x)=1\lor k(x)=1}.$$
% We have that $\mu(X)\le 19\mu(k)$.

Now, we return to analyzing the probability that the 4-function Diamond test
rejects $(f,g,h,k)$. This probability is at least
\[ \Pr_{(a,x,b)\sim\DP}[k(b)=1 \land f(a)=g(\phi_x(a,b))=h(\phi_x(b,a))=0]. \] 
We can lower bound this probability by 
\[ \mu(k)-\Pr_{a\sim\F_2^{d},b\sim\T_p(a)}[k(b)=f(a)=1]-\Pr_{(a,x,b)\sim\DP}[k(b)=g(\phi_x(a,b))=1]-\Pr_{(a,x,b)\sim\DP}[k(b)=h(\phi_x(b,a))=1]. \] 
Note that if $a\sim \F_2^{d},b\sim\T_p(a)$ then $\phi_x(a,b)$ is distributed as
 $\T_{(1+p)/2}(a)$
Simplifying we obtain:
\begin{equation}
  \label{eq:getreadyforhyper}
\mu(k)-\Pr_{a\sim\F_2^{d},b\sim\T_p(a)}[k(b)=f(a)=1] -
\Pr_{a\sim\F_2^{d},b\sim\T_{(1+p)/2}(a)}[k(b)=g(a)=1] - \Pr_{a\sim\F_2^{d},b\sim\T_{(1+p)/2}(a)}[k(b)=h(a)=1].
\end{equation}
Now, by \cref{lem:modifiedhyper} we can lower bound \cref{eq:getreadyforhyper} by
\begin{equation}
  \label{eq:onemore}
\mu(k)- (\mu(k)\mu(f))^{1/(1+|p|)} - (\mu(k)\mu(g))^{1/(1+(1+p)/2)} -
(\mu(k)\mu(h))^{1/(1+(1+p)/2)}.
\end{equation}
Recalling our bounds on $\mu(f),\mu(g),\mu(h)$ we can lower bound \cref{eq:onemore} by
\begin{equation}
  \label{eq:almostthere}
\mu(k)[1- 6\mu(k)^{2/(1+|p|)-1} - 12\mu(k)^{4/(p+3)-1}].
\end{equation}
Observe that the exponents on $\mu(k)$ in \cref{eq:almostthere} are bounded
above $1$ for all $p\in (-1,1)$. Thus, there is some constant $c_p$ (dependent
only on $p$ ) such that if $\mu(k)\le c_p$ then the rejection probability in
\cref{eq:almostthere} is at least $\mu(k)/2$, as desired.
\end{proof}

\subsubsection{Soundness of the $p$-biased Diamond Test}
Equipped with \cref{thm:dichotomy} we can now give the inductive analysis of the Diamond test's soundness. Ultimately we would like to show that if the 4-function Diamond test rejects $(f,g,h,k)$ with probability exactly $\eps$, then $f,g,h,k$ are all $O(\eps)$-close to affine.
So far, we have shown that if $(f,g,k,h)$ is rejected by the $4$-function
Diamond test with probability $\eps$, then $f,g,k,h$ are each \emph{either}
$c_p$-far from affine, or $2\eps$-close to affine.
We now rule out the possibility that $f$ is $c_p$-far from affine, but that the
test rejects with arbitrarily small probability.
\begin{theorem}\label{thm:induct}
Fix $p\in (-1,1)$. Let $c_p$ be the constant from \cref{thm:dichotomy}.
There is a constant $\delta_p$ such that the following holds.
Fix $d\in \N$, and functions $f,g,h,k: \F_2^{d}\to \F_2$. Suppose $f$ is
$c_p$-far from affine. Then, the $p$-Biased 4-function Diamond test rejects $(f,g,h,k)$
with probability at least $\delta_p$.
\end{theorem}

Towards the proof of \cref{thm:induct}, we will require the following Lemma from \cite{optimalreedmuller}.

\begin{lemma}[Lemma 12 of \cite{optimalreedmuller}]\label{fact:nocloserestrictions}
There exists a constant $M_p\in\N$ (dependent on $p$, but independent of $d$) such
that the following holds.
If $f:\F_2^{d}\to\F_2$ has $M_p$ many $1$-variable restrictions $f_{i,\sigma}$
which are $c_p/2$-close to affine, then $f$ is $c_p$-close to affine.
\end{lemma}
In \cite{optimalreedmuller}, the above lemma is actually bounds the number of hyperplanes on which $f$ can be close to affine, but we note that $1$-variable restrictions are also hyperplanes, and so the lemma stated above is holds as well. We state it as such as it better suits our application.

\begin{proof}[Proof of \cref{thm:induct}]
Given a function $f:\F_2^{d}\to \F_2$, coordinate $i\in [d]$, and value
$\sigma\in \F_2$, define the 1-variable restriction $f_{i,\sigma}:\F_2^{d-1}\to \F_2$ to be $f\mid_{x_i=\sigma}$.

Let $M_p$ denote the constant from \cref{fact:nocloserestrictions}.
Define $\delta_p=\min(c_p/2, (p/8)^{M_p})$.

We will prove the theorem by induction on the dimension $d$.
Our base case is $d\le M_p$.
If $d\le M_p$ then by \cref{lem:basecase} the 4-function Diamond test
rejects $(f,g,h,k)$ with non-zero probability since $f$ is not affine.
But, the smallest non-zero probability that the test could possibly reject with
is $(p/8)^d\ge (p/8)^{M_p}\ge \delta_p$.

Now, fix $d> M_p$, and assume the theorem for functions on $\F_2^{d-1}$.
Because $f$ is $c_p$-far from affine, \cref{fact:nocloserestrictions} implies
that there at most $M_p$ many 1-variable restrictions of $f$ which are
$c_p/2$-close to affine.
Thus, there is some $i\in [d]$ such the restrictions $f_{i,0}$ and $f_{i,1}$ are
both $c_p/2$-far from affine.

To analyze the probability that the 4-function Diamond test rejects $(f,g,h,k)$,
we consider a partition of the probability space into $8$ disjoint events. 
The events are the value in $\F_2^{3}$ that our sampled $(a_i,b_i,x_i)$ takes.
Now, consider the probability that the 4-function Diamond test rejects
$(f,g,h,k)$, conditional on $(a_i,b_i,x_i)=(\alpha,\beta,\xi)$ for some $\alpha,\beta,\xi$.
Conditional on this event, we will sample $a,b,x\in \F_2^{d-1}$ and check:
\[ f_{i,\alpha}(a)+g_{i,\phi_\xi(\alpha,\beta)}(\phi_x(a,b)) =
h_{i,\phi_\xi(\beta,\alpha)}(\phi_x(b,a))+k_{i,\beta}(b). \] 
This is precisely a 4-function Diamond test on $(d-1)$-dimensional functions.
Now we consider two cases.\\
\textbf{Case 1: $f_{i,\alpha}$ is $c_p$-far from affine}. \\
Then by the inductive hypothesis this $(d-1)$-dimension test will reject with
probability at least $\delta_p$.\\
\textbf{Case 2:} $\dist(f_{i,\alpha}, \mathsf{affine})\in [c_p/2, c_p]$.\\
Then, by \cref{thm:dichotomy} this $(d-1)$-dimensional diamond test rejects with
probability at least $c_p/2\ge \delta_p$.

We have seen that in all cases, the lower dimensional 4-function Diamond tests
reject with probability at least $\delta_p$.
Thus, the actual 4-function Diamond test rejects with probability $\delta_p$ as well.
\end{proof}

Combining \cref{thm:dichotomy} and \cref{thm:induct} we have get the following corollary.
\begin{corollary}\label{cor:4fun}
Fix $p\in (-1,1)$.
If $(f,g,h,k)$ passes the $p$-Biased 4-function Diamond test with probability
$1-\eps$, then $f,g,h,k$ are each $O_p(\eps)$-close to affine. 
\end{corollary}
\begin{proof}
    This result follows immediately from  \cref{thm:dichotomy} and \cref{thm:induct}.
\end{proof}
% \todo{In fact, fgjk should all be close to the same affine function modulo pushing +1's around. But Im not going to write this down right now.}
We can now conclude the proof of \cref{cor:1fun} and establish soundness for the $p$-biased Diamond test.

\begin{proof}[Proof of \cref{cor:1fun}]
    The result follows from \cref{cor:4fun} by setting $f = g = h = k$.
\end{proof}
% In fact, in the 4-function setting, we can give a slightly stronger conclusion:
% \begin{corollary}
% Fix $p\in (-1,1)$.
% Suppose $(f,g,h,k)$ passes the $p$-Biased 4-function Diamond test with probability $1-\eps$.
% Then, there is a linear function $L$ such that $f,g,h,k$ are all $O_p(\eps)$-close to either $L$ or $L+1$.
% \end{corollary}
% \begin{proof}
%  Fix such $f,g,h,k$.
%  By a union bound and \cref{fact:fliperoo} (just as in \cref{lem:4basecase}) we have:
%  there exists constants $\alpha,\beta$ such that $k$ is $2\eps$-close to $f+\alpha$, and $h$ is $2\eps$-close to $g+\beta$.
% By \cref{cor:4fun} there exist affine functions $F,G$ such that $f$ is
%  $O_p(\eps)$-close to $F$ and $g$ is $O_p(\eps)$-close to $G$.
% Then by a union bound:
% $$\Pr_{a,x\sim\F_2^{d},b\sim\T_p(a)}[F(a)+F(b)=G(\phi_x(a,b))+G(\phi_x(b,a))+\alpha+\beta]>1-O_p(\eps).$$
% Now, observe that 
% $$G(\phi_x(a,b))+G(\phi_x(b,a)) = G(a)+G(b).$$
% Thus we have
% $$\Pr_{a\sim\F_2^{d},b\sim\T_p(a)}[F(a+b)=G(a+b)+\alpha+\beta]>1-O(\eps).$$
% Thus, $f,g,h,k$ are all $O_p(\eps)$-close to either $F$ or $F+1$.
% \end{proof}



==> introduction.tex <==
\section{Introduction}
\paragraph{Background}

In this paper we consider several \defn{property testing} questions (see
\cite{gold_intro} for an introduction to the subject).
In property testing, we have query access to a function $f$, and want to
\defn{test} whether $f$ has a property $\mc{P}$.
For example, the property could be could be ``$f:\F_2^{d}\to \F_2$ is linear''. 
We would like to determine whether $f$ has property $\mc{P}$ using a small
number of queries, ideally where the number of queries required does not scale
with the size of $f$'s domain.
Already for linearity we can see that this goal is unattainable as stated: to
determine whether $f$ is linear, we must know the value of $f$ at each point in
the domain. 
The solution is to make the problem easier.
Instead of building an algorithm to distinguish between functions that have
$\mc{P}$ and functions that do not, we set our goal to be distinguishing between
functions that have property $\mc{P}$ and functions which are \emph{far} from
having property $\mc{P}$.
We say the \defn{distance} from $f$ to property $\mc{P}$ is the fraction of
inputs $x$  on which we would need to change the value $f(x)$ in order to obtain
a function $f' \in \mc{P}$.

This definition of testing gives rise to a rich class of problems that have been
explored over the past 35 years.
\todo{list some questions. e.g., low degree, linearity, direct sum, direct product}

In this paper consider several \defn{property testing} questions.
In property testing, we have query access to a function $f$, and want to
\defn{test} whether $f$ has a property $P$.

% Property testing is a subfield of theoretical computer science interested in discerning whether an object $f$ satisfies some property $P$ through making queries about $f$. In this paper, we focus specifically on property testing for functions with finite domains, where a property $P$ is simply some class of functions. We usually wish to design tests with as low query complexity as possible, with the number of queries often being far below the number required to exactly determine $f$ itself.
% \todo{this is not true of all properties (??)}
\todo{pcp!}

In general, discerning exactly whether $f$ has a property $P$ (such as being linear) often requires querying $f$ at nearly all its values, so we instead allow our test a certain margin of error. Defining the distance between two functions $f,g$ on the same (finite) domain to be $\Pr_x[f(x) \neq g(x)]$, with $x$ chosen uniformly at random from the domain, we say that a \defn{one-sided tester} for $P$ is a test with two properties: \emph{completeness} and \emph{soundness}. Completeness refers to the success rate when $f$ does have property $P$; for one-sided testers we require the test to accept $f$ deterministically. Soundness refers to the probability the test rejects for any $f$ that is $\eps$-far from $P$ (which means $\dist(f,g) \geq \eps$ for all $g \in P$); we desire this to be a nontrivial probability, often $O(\eps)$.

In general, we are interested in constructing tests for global properties, for example linearity (there exists $c$ such that $f(x) = c \cdot x$ for all $x$) or parity (that $f(x) = f(-x)$ for all $x$). This means that good few-query tests give a connection between a local property with high probability and closeness to a global property.

In this paper we are interested specifically in property testing for Boolean functions over grids, functions $f: [n_1] \times [n_2] \times \cdots \times [n_d] \to \F_2$.
A foundational result in this area is a linearity test first proposed by Blum, Luby, and Rubinfield~\cite{BLR} for a function $f: \F_2^d \to \F_2$. Our goal is to test if $f$ is far from the set of linear functions $g(x) = c \cdot x$ for some vector $c \in \F_2^d$. It is simple to verify that $f$ is linear if and only if $f(x+y) = f(x) + f(y)$ for all $x,y \in \F_2^d$, which yields the test:

\begin{test}[BLR linearity test]\label{test-blr-linearity}
    Select $x, y \in \F_2^d$ independently and uniformly at random. Accept if $f(x) + f(y) = f(x+y)$, and reject otherwise.
\end{test}

It is clear from the above that when $f$ is linear, the test is guaranteed to accept. On the other hand, one can show that when $f$ is $\eps$-far from linear, the test rejects with a $1-\eps$ probability (see \Cref{theorem-blr-linearity}). Linearity testing naturally extends to \defn{affinity testing}, corresponding to the set of affine functions $f(x) = a\cdot x + b$. For instance, one can employ identical arguments to show a version of the BLR test for affinity:

\begin{test}[BLR affinity test]\label{test-blr-affinity}
    Select $x,y,z \in \F_2^d$ independently and uniformly at random. Accept if $f(x) + f(x+y) + f(x+z) + f(x+y+z) = 0$.
\end{test}

A generalization of affinity from the hypercube $\F_2^d$ to the grid $[n_1] \times \cdots \times [n_d]$ is the \emph{direct sum}. We say that $f: [n_1] \times \cdots \times [n_d]$ is a direct sum if there exist functions $L_i: [n_i]  \to \F_2$ (for $1 \leq i \leq d$) such that $f(x) = \sum_i L_i(x_i)$. Note that, unlike the hypercube $\F_2^d$, this grid possesses no additive structure.
Testing whether a given function is a direct sum was first studied by David et. al. in~\cite{david2015direct}, though in the somewhat different domain over slices of the hypercube (i.e., strings in $\{0,1\}^d$ with Hamming weight $k$). The aformentioned case of the full hypergrid was studied by Dinur and Golubev in~\cite{di19}, who gave two natural tests for direct sum testing: the \emph{Square in Cube} test and the \emph{Shapka Test}, which we will be giving further analysis of in \cref{sec:subcube} and \cref{sec:correction}. They also proposed a third test which we will refer to as the \emph{diamond} test; we will be analyzing the validity of this test, though only over $\F_2^d$, in \cref{sec:diamond}.

In the later sections of this paper we will consider the generalization of the class of linear functions to the class of $k$-juntas, a problem otherwise known as junta-degree testing. Formally, a function $f: [n_1]\times\cdots\times[n_d] \to \F_2$ is a $k$-junta if it depends on $k$ of the $d$ variables, and $f$ has junta-degree $k$ if it can be expressed as the sum of $k$-juntas. Questions regarding junta-degree testing have been studied in~\cite{srinivasan2018local} and \cite{amireddy2023low}. \todo{any results from these to specifically cite?}

% tbh i think this might be better in the conclusion?
% \paragraph{Open Questions}
% \todo{Do more with the Junta-degree stuff. Proving the multi-DP fact is probably the
% highest priority thing here. Is there a more direct analysis of the Diamond test / Diamond in Cube test?}

\section{An Exposition of Some Basic Results in Property Testing}
\todo{
Honestly I kind of propose cutting this section and / or moving it to an appendix (even for spur).
The magic square is very cool, but I don't think it's that relevant for the rest of the paper.
}

In this section, we present a classic property testing result (an analysis of
the BLR linearity test), with the goal of giving a reader who is unfamiliar with
the area a sense of some techniques used in property testing. If the reader is
already acquainted with the basics of property testing, they can freely skip
this section.

% We begin by presenting two analyses of
% \Cref{test-blr-linearity}. (These are both analyses of soundness; completeness
% is obvious for this test.) The first one reconstructs the linear function which
% our given function $f$ is $\eps$-close to.

\begin{theorem}
If a function $f: \F_2^d \to \F_2$ is $\eps$-close to linear, then
\cref{test-blr-linearity} passes with probability at least $1-5\eps$.
\end{theorem}
\begin{proof}
    Let $g(x)$ be the majority vote of $f(a) + f(x+a)$ across all $a$. The main idea is to show that $g$ is linear, and $f$ is close to $g$; as such, $g$ can be thought of as the ``corrected'' version of $f$. 
    % \todo{thoughts on calling $g$ like $\tilde{f}$ instead or something}\todo{do it if you want!}

    \begin{claim}
        $\Pr_{x,y}[f(a)+f(x+a) = g(x)] \geq 1-4\eps$, i.e.\ the majority vote is an actual majority.
    \end{claim}
    \begin{proof}
        Consider $a,b,y$ chosen randomly. Construct the following square:
    
        \begin{center}
            \begin{tabular}{|c|c|c|}
                \hline
                $x$   & $x+a$   & $a$       \\
                \hline
                $x+b$ & $y$     & $x+y+b$   \\
                \hline
                $b$   & $x+y+a$ & $x+y+a+b$ \\
                \hline
            \end{tabular}
        \end{center}
    
        The second and third columns and rows can all be seen to be BLR tests, so by union bound they all pass with probability $1-4\eps$ or more. Assuming all pass, add the equations for the columns and subtract the equations for the rows to obtain $\Pr_{a,b,y}[f(a) + f(x+a) = f(b) + f(x+b)] \geq 1-4\eps$. Eliminate $y$, recall that $g(x)$ is the majority of $f(a) + f(x+a)$, and conclude.
    \end{proof}
    
    \begin{claim}
        $g(x)$ is linear.
    \end{claim}
    \begin{proof}
        Fix arbitrary $x,y$. Pick $a,b$ randomly; then consider the square
    
        \begin{center}
            \begin{tabular}{|c|c|c|}
                \hline
                $x+a$ & $y+b$   & $x+y+a+b$ \\
                \hline
                $x+b$ & $y$     & $x+y+b$   \\
                \hline
                $b$   & $x+y+a$ & $x+y+a+b$ \\
                \hline
            \end{tabular}
        \end{center}
    
        By the previous claim, the probabilities that $g(x) = f(x+a) + f(a)$ and $g(y) = f(y+b) + f(b)$ and $\Pr[g(x+y) = f(x+y+a+b) + f(a+b)]$ are all at least $1-4\eps$. Meanwile by BLR, the probabilities that $f(x+a) + f(y+b) = f(x+y+a+b)$ and $f(a) + f(b) = f(a+b)$ are both at least $1-\eps$. By union bound (assuming $\eps$ is small) we obtain $g(x) + g(y) = g(x+y)$.
    \end{proof}
    
    \begin{claim}
        $\Pr_x[f(x) = g(x)] \geq 1-5\eps$, i.e.\ $f$ almost always agrees with $g$.
    \end{claim}
    \begin{proof}
        We can simply write $\Pr_x[g(x) \geq f(x)] \geq \Pr_{x,y}[g(x) = f(x) = f(a) + f(x-a)]$, and by union bound (BLR with the first claim) this is at least $1-5\eps$.
    \end{proof}
\end{proof}

% An analysis using Fourier-analytic methods \todo{do we even need this? we don't do any fourier analysis in the rest of the paper...}
% oh i forgot that the "fourier-analytic fact" equivalent to the diamond test isn't actually fourier analytic. sure -EY
% \todo{is it ok if I start editting intro? you can keep going on this exposition stuff.}


==> junta-degree-d.tex <==
\section{Junta-Degree $k$ Testing}

In this section, we consider the generalization of direct sum testing to
\textbf{junta-degree $k$} testing, i.e., testing whether $f$ is the sum of
functions which only look at $k$ bits of the input at a time (direct sum being
the case $k=1$). Using a similar technique to the Affine on Subcube test, we
show how to test whether a function $f: S_1\times \cdots \times S_d \to \F_q$,
for any $2$ element sets $S_1,\ldots, S_d\subseteq \F_q$, is a restriction of a
degree $k$ polynomial over $\F_q$ to an asymmetric grid. Such a test was already
given in by Bafna, Srinivasan, Sudan \cite{srinivasan2018local}; our test
improves the query complexity of this previous work. This complements recent
work in \cite{amireddy2023low} by Amireddy, Srinivasan and Sudan which shows
that this is impossible if the sets $S_i$ are instead allowed to be of size $3$.

Formally, we say that a function $f:[n]^d\to \F_q$ is Junta-degree $k$ if there exist
functions $g_S: [n]^{S}\to \F_q$ for each $S\in \binom{[d]}{k}$ such that 
\[ f(x) = \sum_{S} g_S(x_S). \] 
An important ingredient in our analysis will be a generalization of the
\cite{dinur2014direct}'s direct product test (\cref{test:dp}) to a \defn{$k$-direct product} test.
We say that $F:[n]^d \to \F_q^{\binom{[d]}{\le k}}$ is a $k$-direct product if there
are functions $\setof{G_S}{S\in \binom{[d]}{k}}$ so that for each $S\in
\binom{[d]}{k},x\in [n]^d$, we have $F_S(x)=G_S(x_S)$.
We conjecture:
\begin{conjecture}\label{conj:highdimdp}
Fix integers $n,d,k$.
Let $F: [n]^d \to \F_q^{\binom{[d]}{\le k}}$, satisfy the following agreement condition:
$$\Pr_{b,b'\sim \T_{1/2}(b)} \left[F_{S}(b) = F_{S}(b') \quad \forall S\in \binom{[d]}{\le k} \mid b_S = b'_S\right] > 1-\eps.$$ 
Then, there are functions $\setof{g_S:[n]^{S}\to \F_q}{S\in \binom{[d]}{\le k}}$ such that 
$$\Pr_{b}\left[F_S(b) = g_S(b_S) \quad\forall S\in \binom{[d]}{\le k}\right] > 1-O(\eps).$$
\end{conjecture}
For $n>2$ we are not aware of a proof of this conjecture in the literature,
although we believe that techniques in the literature could be adapted to prove
this result. \cref{conj:highdimdp} is quite natural, and we propose resolving it
as a direction for future research. Our work provides motivation for proving
\cref{conj:highdimdp}: we believe that if \cref{conj:highdimdp} were resolved,
our techniques could be adapted to give a simple tester for junta-degree $k$ for any $n$.
For the case of $n=2$ however, \cref{conj:highdimdp} follows immediately from
work by Dinur et al. \cite{dinur2017agreement}:
\begin{fact}[Theorem 1.2 of \cite{dinur2017agreement}]\label{fact:multidp}
\cref{conj:highdimdp} is true for $n=2$.
\end{fact}
Thus, we will be content to analyze our test for the case $n=2$ which is already interesting.
In particular, one reason why the case $n=2$ is interesting is the following observation:
\begin{proposition}\label{prop:juntadegVSdeg}
Fix $\F_q,d$ and 2-element sets $S_1,\ldots, S_d\subseteq \F_q$.
If $f:\prod_i S_i \to \F_q$ is junta-degree $k$, then $f$ can be extended to a
degree $k$ polynomial on $\F_q^{d}$, and in particular such a polynomial where
the power of each variable in each monomial is at most $1$.
\end{proposition}
\begin{proof}
Let $S_i = \set{s_{i,0},s_{i,1}}$.
Then, we can write $f$ as 
\[ f(x) = \sum_{y\in \F_2^{d}} f(y)\cdot \prod_i (x_i - s_{i,y_i}) \prod_i
(s_{i,y_{i+1}} - s_{i,y_{i}})^{-1}.\] 
Now, we can interpret this as a polynomial over $\F_q^{d}$.
\end{proof}

Generalizing the Affine on Subcube test, we propose the following test for testing junta-degree $k$:
\begin{test}
  Sample $a,b\in [n;d]$ randomly. Run a degree $k$ tester on $x\mapsto f(\phi_x(a,b))$.
\end{test}
This test is complete: the restriction of a junta-degree $k$ function to a subcube
is a degree $k$ polynomial. We will show that for $n=2$ the test is sound.
First, we need the following lemma.

\begin{lemma}\label{lem:distancetozero}
Fix $d,k,\F_q$ and 2-element sets $S_1,\ldots, S_d\subseteq \F_q$. Let $x\sim
\mc{D}$ be a distribution on $\prod_{i} S_i$ where the values $x_i$ are
independent and for each $s\in S_i$, $x_i$ takes on value $s$ with probability
at least $.1$. 
Then, if $f$ is a non-zero junta-degree $k$ function on $\prod_i S_i$ we have
\[ \Pr_{x\sim \mc{D}}[f(x)\neq 0] \ge 1/10^k. \] 
\end{lemma}
\begin{proof}
We induct on the degree $k$.
The base case $k=1$ is trivial. 
Assume the claim for functions of junta-degree $k-1$. 
Now, fix a function $f:\prod_i S_i\to \F_q$ of junta-degree $k$, and use
\cref{prop:juntadegVSdeg} to view $f$ as a degree $k$ polynomial on $\F_q^{d}$
where the exponent of each variable in each monomial is at most $1$.

Let $z$ be a variable that appears with a non-zero coefficient in some monomial
of $f'$. Re-index the variables so that $z$ is the $d$-th variable.
Let $\alpha,\beta$ be the two possible settings of $z$, and let $p\in [.1,.9]$
be the probability that $z=\alpha$ under $(y,z)\sim\mc{D}$.
Then, we have
\[ f(y,z) = zg(y) + h(y), \] 
where $g$ a non-zero degree $k-1$ polynomial.
Define 
\[ \psi = \Pr_{(y,z)\sim \mc{D}} [g(y)\neq 0 \land \alpha g(y)\neq h(y)], \] 
\[ \psi' = \Pr_{(y,z)\sim \mc{D}} [g(y)\neq 0 \land \beta g(y)\neq h(y)]. \] 
Observe that 
$$\psi+\psi' \ge \Pr_{(y,z)\sim \mc{D}}[g(y)\neq 0].$$
Because $g$ is a degree $k-1$ polynomial we have, by the inductive hypothesis,
that
\[ \Pr_{(y,z)\sim \mc{D}} [g(y)\neq 0] \ge 1/10^{k-1}. \] 
We can bound the chance of $f$ being zero as follows:
\begin{align*}
\Pr_{(y,z)\sim \mc{D}} [f(y,z)\neq 0] 
&\ge p\psi + (1-p)\psi'  \\
&\ge \mu(k) \cdot (p\psi/\mu(k) + (1-p)(1-\psi/\mu(k)) )  \\
&\ge \mu(k) \cdot \min(p,1-p) \\
&\ge  1/10^{k}.
\end{align*}
\end{proof}

Now, we show that for $n=2$ the test is sound.
\begin{theorem}
Fix $q,k,d\in \N$, and let $n=2$. Suppose the expected distance to degree $k$
functions of the restriction of $f:[n]^d\to \F_q$ to a random subcube is $\eps$.
Then $f$ is $C_{k,q}\eps$-close to a direct sum for some constant $C_{k,q}$
depending on the degree $k$ test and the field size, but not on $d$.
\end{theorem}
\begin{proof}
In this proof we will use $O(\cdot)$-notation to hide constants that are allowed to
depend on $k,q$, but not on $d$.
For each $a,b$, let $F^{ab}:\F_2^{d}\to \F_q$ denote the closest degree $k$
function to $x\mapsto f(\phi_x(a,b))$.
\todo{does this even make sense}
 Define
\begin{equation}\label{epsab:final}
\eps_{ab} = \Pr_{x}[f(a_xb) \neq F^{ab}(x)].
\end{equation}
By averaging we have $\E_{ab}[ \eps_{ab} ] = \eps.$

\begin{lemma}\label{lem:closemultidp}
$b\mapsto F^{ab}$ is $O(\eps_a)$-close to a $k$-direct product.
\end{lemma}
\begin{proof}
Given $b,b'$, define distribution $x\sim \mc{D}_{bb'}$ on $\F_2^d$ as follows:
\begin{quote}
$x_i=0$ for all $i\in \Delta(b,b')$,
and, if $b_i=b_i'$ then $x_i=1$ with probability $2/3$ and $0$ else.
\end{quote}
Now, observe that if we sample $b'\sim \T_{1/2}(b), x\sim \mc{D}_{bb'}$ then the
values $x_i$ are independent uniformly random bits.
However, if we choose $b',x$ like this then we guarantee
\[ \phi_x(a,b)=\phi_x(a,b'). \] 
Now, performing a union bound on \cref{epsab:final}, gives 
$$ \Pr_{b\sim[n]^{d},b'\sim \T_{1/2}(b),x\sim \mc{D}_{bb'}} [F^{ab}(x) =f(a_xb)
= f(a_xb') = F^{ab'}(x)] \ge 1-2\eps_{a}. $$
Let 
$$ \delta_{abb'} =  \Pr_{x\sim X_{bb'}} [F^{ab}(x)\neq F^{ab'}(x)]. $$
Write
\[F^{ab}(x) = \sum_{S \in \binom{[d]}{\le k}} F^{ab}_S \prod_{i\in S}x_i. \] 
Define $$A_{bb'} = \setof{S\in \binom{[d]}{\le k}}{b_i = b_i' \forall i\in S}.$$
By \cref{lem:distancetozero} we have that if $\delta_{abb'} < 1/3^{k}$, then for
all $S\in A_{bb'}$, $F^{ab}_S = F^{ab'}_S$.
Now, by Markov's Inequality we have that 
$$ \Pr_{b,b'\sim D_{b}}[\delta_{abb'}>3^{-k}] \le 3^{k}\mathbb{E}_{b,b'}[\delta_{abb'}] < O(3^{k}\eps_a). $$
From this we conclude
$$ \Pr_{b,b'\sim D_{b}} [ \forall S\in A_{bb'}, F^{ab}_S = F^{ab'}_S] \ge 1-O(3^{k}\eps_a). $$
Then, applying \cref{fact:multidp} finishes the proof of the lemma.

\end{proof}

It is helpful to restate this as follows:
\begin{corollary}\label{cor:kdirectsum}
For each $a$, there exists $G^a = \setof{G^a_S:[n]^S\to \F_2}{S\in \binom{[d]}{\le k}}$
such that 
$$\Pr_{b\sim T_{1/2}(a)}\left[f(b) = \sum_S G^a_S(b_S) \right] > 1-O(\eps_a).$$
\end{corollary}
\begin{proof}
Performing a union bound on \cref{epsab:final} and \cref{lem:closemultidp} we have
$$\Pr_{a,x,b}\left[f(a_xb) = \sum_S G^a_S(b_S) \prod_{i\in S} x_i \right] > 1-O(\eps_a),$$
where $G^a_S$ is the closest $k$-direct product to $b\mapsto F^{ab}$.
Then, we define
$$\widetilde{G^a}_S((a_xb)_S) = G^a_S(b_S) \prod_{i\in S} x_i.$$
This is well defined because if $\prod_{i\in S} x_i = 0$, then we give the value
$0$, and if $x_i = 1$ for all $i\in S$ then $(a_xb)_S = b_S$.
Then, 
$$\Pr_{b\sim \T_{1/2}(a)}\left[f(b) = \sum_S \widetilde{G^a_S}(b_S) \right] > 1-O(\eps_a).$$
\end{proof}
In \cref{cor:kdirectsum} we have shown that \emph{locally} our function $f$ is close to junta-degree $k$.
To finish, we will show that these local junta-degree $k$ functions agree.
First, we need the following lemma about junta-degree $k$ functions.

\todo{just get rid of the n's in this stuff}
\begin{lemma}
$$ \Pr_{a,b}[G^a = G^b]> 1-O(n\eps). $$ 
\end{lemma}
\begin{proof}
Let $B_{1/4}(a)$ be the set of points that disagree with $a$ on
at most $1/4$ of their coordinates.
Fix $a,b\in B_{1/4}(a)$.
Let $r\ge 3/4$ be the fraction of coordinates on which $a_i,b_i$ agree.
Define distribution $y\sim \mathcal{D}$ as follows:
\begin{itemize}
\item If $a_i=b_i$, then $y_i = a_i$ with probability $(1/2-1/(2n))/r+1/n$ and
sample it uniformly randomly from $[n]\setminus \set{a_i}$ otherwise.
\item If $a_i\neq b_i$, then sample $y_i$ uniformly randomly.
\end{itemize}
We now make some observations about this distribution.
First, observe that 
\[ \Pr[y_i = a_i \mid a_i = b_i] = (1/2-1/(2n))/r+1/n  \le 2/3. \] 
The fact that this probability is less than $1$ makes our distribution well
defined, while the fact that this probability is bounded away from $1$ will be
important later.
Second, observe that at each coordinate $i$, 
$$\Pr[a_i = y_i] = \Pr[b_i = y_i] = r\cdot \left( (1/2-1/(2n))/r+1/n \right) +
(1-r)/n  = \frac{1}{2} + \frac{1}{2n}.$$ 
That is, $y$ has the same distribution as $\T_{1/2}(a)$ (if we
don't look at $b$) and as $\T_{1/2}(b)$ (if we don't look at $a$).
Define $g^a(x) = \sum_S G^a_S(x_S)$, where $G^a$ is the $k$-direct product given in \cref{cor:kdirectsum}.
Define 
$$\delta_a = \Pr_{b\sim \T_{1/2}(a)}[g^a(b)\neq f(b)].$$
By \cref{cor:kdirectsum} we have $\delta_a \le O(\eps_a)$.
Then,
$$ \Pr_{y\sim \mathcal{D}}[f(y)\neq g^a(y) \bigvee f(y)\neq g^b(y)]\le \delta_a+\delta_b. $$
By a union bound this means:
$$ \Pr_{c\sim \mathcal{D}}[g^a(c) = g^b(c)]\ge 1-(\delta_a+\delta_b). $$
Now, because $g^a,g^b$ are direct sums, by \cref{lem:distancetozero} we have
that if $\eps_a+\eps_b < (.1/n)^k$, then 
$$ g^a = g^b. $$ 
Of course, by Markov's inequality we have:
$$ \Pr_{a,b\in B_{1/4}(a)}[\eps_a+\eps_b<(.1/n)^k]>1-O((10n)^k\eps). $$ 
Thus, 
$$ \Pr_{a,b\in B_{1/4}(a)}[g^a=g^b] > 1-O((10n)^k\eps). $$ 
Finally, taking a sequence $a_1,a_2,a_3,a_4,a_5$ where $a_i,a_{i+1}$ are each
$3/4$ correlated but  $a_1,a_5$ are just random independent points, and using a
union bound, we have that:
$$ \Pr_{a,b}[g^a = g^b] > 1-O((10n)^k\eps). $$ 
\end{proof}

Now we finish proving the theorem.
$$ \Pr_{a,b,c\sim T_{1/2}(b)} [g^a \neq g^c  \bigvee  g^c(b)\neq f(b)] \le O((10n)^k\eps). $$ 
Thus, 
$$ \Pr_{a,b}[g^a(b) = f(b)] > 1-O((10n)^k\eps).$$ 
Then, by the probabilistic method we can choose $a$ such that $f$ is
$O((10n)^k\eps)$ close to the junta-degree $k$ function $g^a$.
    
\end{proof}



==> notes/DEPRECATED_square_in_cube.tex <==
\section{Square in Cube}\label{sec:squarecube}

\begin{remark}
Their analysis of this test is \textbf{very wrong}. 
I will endeavor to give correct analysis below.
\end{remark}

Throughout the analysis we will use the following basic fact from probability theory many times:

\begin{fact}
Let event $E$ be a function of $x,b$.
Suppose that for all $b$, $\Pr_x[E(x,b)]> \rho_b.$\\
Then, $\Pr_{x,b}[E(x,b)] > \mathbb{E}[\rho_b]$.
\end{fact}

Define $S_x(a,b)$ to be the vector obtained by taking $a_i$ whenever $x_i = 0$ and $b_i$ whenever $x_i = 1$. 
We can also write this as $a\bar{x}+bx$ where the vector multiplication is done element-wise.
Define $\Delta(a,b) \subseteq [d]$ to be the set of indices where $a,b$ differ. 

\begin{definition}[Square in Cube Test]
Sample random $a,b\in [n]^d$ and $x,y\in \mathbb{F}_2^{d}$ and test:
$$ 
f(S_0(a,b)) + f(S_x(a,b))+ f(S_y(a,b))+f(S_{x+y}(a,b))=0.
$$ 
\end{definition}

Clearly we have:
\begin{proposition}
    If $f$ is $\eps$ close to a direct sum, then the Square in Cube Test passes with probability at least $1-4\eps$.
\end{proposition}

Now we show that the test is sound. 
\begin{theorem}
If $f:[n]^d\to \F_2$ passes the Square in Cube test with probability $1-\eps$, then there is an absolute constant $C<2^{100}$ such that $f$ is $C\eps$-close to a direct sum.
\end{theorem}
\begin{proof}
Let 
$$  \eps_{ab}=\Pr_{x,y}[f(S_0(a,b)) + f(S_x(a,b))+ f(S_y(a,b))+f(S_{x+y}(a,b))\neq0]. $$
Let $\eps_a = \mathbb{E}_b [\eps_{ab}]$. Suppose $f$ passes the Square in Cube test with probability $1-\eps$. Then, $\mathbb{E}_{ab} [\eps_{ab}]=\mathbb{E}_a [\eps_a] = \eps$.
It is valuable to re-express $\eps_{ab}$ as follows:
$$ 
\eps_{ab}=\Pr_{x,y}[(f(a) + f(S_x(a,b)))+ (f(a)+f(S_y(a,b)))\neq f(a)+f(S_{x+y}(a,b))].
$$
For each $(a,b)$, the \textbf{BLR test} implies the existence of a character $I_{ab}\subseteq \Delta(a,b)$ such that
$$
\Pr_x[f(a)+f(S_x(a,b))=\chi_{I_{ab}}(x)]>1-\eps_{ab}.
$$
Let $F_a(b)\in \mathbb{F}_2^{d}$ be the indicator vector for $I_{ab}\subseteq [d]$. 

\begin{lemma}
$F_a(b)$ is close to a direct product $(g_{1}(a,b_1),\dots,g_d(a,b_d))$
\end{lemma}

\begin{proof}
Define distribution $b'\sim D_{b}, b'\in [n]^d$ as follows: 

\begin{quote}
Sample $b'$ uniformly randomly, conditional on having $b_i'= b_i$ hold for exactly $3d/4$ of $i\in [d]$. 
\end{quote}

Define distribution $x\sim X_{bb'},x\in \mathbb{F}_2^d$ as follows:
\begin{quote}
$x_i=0$ for all $i\in \Delta(b,b')$,
and, if $b_i=b_i'$ then $x_i=1$ with probability $2/3$ and $0$ else.
\end{quote}

Observe: For any $x_{0}\in \mathbb{F}_2^d$, $\Pr_{b,b'\sim D_{b},x\sim X_{bb'}}[x=x_{0}]=1/2^d$. 
That is, $x$ is uniformly distributed, and pairwise independent of $b,b'$, although of course the triple $(x,b,b')$ is dependent. 
By construction, $S_x(a,b) = S_x(a,b')$ (whenever $b_i,b_i'$ differ, we choose $a_i$).
Then, by a union bound (and averaging away $b$ in our earlier expression) we have that 
$$
\Pr_{b,b'\sim D_{b},x\sim X_{bb'}} [\chi_{F_a(b)}(x) =f(a)+f(S_x(a,b)) = f(a)+f(S_x(a,b')) = \chi_{F_a(b')}(x)] > 1-2\eps_{a}.
$$
Let 
$$
\delta_{abb'} =  \Pr_{x\sim X_{bb'}} [\chi_{F_a(b)\oplus F_a(b')}(x) \neq 0].
$$
Let $\overline{\Delta}(b,b')$ denote the set of indices $i$ where $b_i=b_i'$. For vector $x\in \mathbb{F}_2^d$, and set $S\subseteq [d]$, let $x\mid_S$ denote the restriction of $x$ to coordinates $S$. Then,

\begin{claim}
If $\delta_{abb'}<1/3$ then $F_a(b)\mid_{\overline{\Delta}(b,b')}= F_a(b')\mid_{\overline{\Delta}(b,b')}$.
\end{claim}
\begin{proof}
Assume for sake of contradiction that there exists  $i\in \Delta(F_a(b), F_a(b')) \cap \overline{\Delta}(b,b')$.\\
Sampling $x\sim X_{bb'}$ we have a $1/3$ chance of $x_i$ being $0$ and a $2/3$ chance of $x_i$ being $1$, independent of the values of $x_j$ for $j\neq i$.\\
But then $\chi_{F_a(b)\oplus F_a(b')}(x)$ doesn't take on any value in $\mathbb{F}_2$ with probability greater than $2/3$, contradicting $\delta_{abb'}<1/3$.\\
Thus, $\Delta(F_a(b), F_a(b')) \cap \overline{\Delta}(b,b') = \varnothing$.
\end{proof}

Now, by Markov's Inequality we have that 
$$
\Pr_{b,b'\sim D_{b}}[\delta_{abb'}>1/3] \le 3\mathbb{E}_{b,b'}[\delta_{abb'}] < 6\eps_a.
$$
From this we conclude
$$
\Pr_{b,b'\sim D_{b}} [F_a(b)\mid_{\overline{\Delta}(b,b')}= F_a(b')\mid_{\overline{\Delta}(b,b')}] > 1-6\eps_a.
$$
By the direct product test we conclude that $F_a(b)$ is $O(\eps_a)$-close to a direct product $(g_1(a,b_1),\dots,g_d(a,b_d))$. 
Combining these facts we have:
$$ 
\Pr_{x,b} \left[ f(a)+f(S_x(a,b)) = \sum_i g_i(a,b_i)x_i \right] > 1-O(\eps_a). 
$$
This concludes the proof of Lemma 1.
\end{proof}

Now we prove the theorem.
Observe that $S_{x}(a,b)=S_{\bar{x}}(b,a)$. Thus, by Lemma 1 and a union bound,
$$
\Pr_{a,b,x} \left[ \sum_{i}g_{i}(a,b_{i})x_{i}= f(a)+f(S_x(a,b))=f(b)+f(S_{\bar{x}}(b,a))=\sum_{i}g_{i}(b,a_{i})\overline{x_{i}} \right]>1-O(\eps).
$$
Define 
$$
\lambda_{ab}=\Pr_x\left[ \sum_i (g_i(a,b_i)+g_i(b,a_i))x_i \neq \sum_i g_i(b,a_i) + f(a)+f(b) \right].
$$
Clearly, if $\lambda_{ab}<1/2$  then we must have 
$$
g_i(a,b_i)=g_i(b,a_i)
$$
for all $i$, and also 
$$
\sum_i g_i(b,a_i)=f(a)+f(b).
$$
By Markov's inequality:
$$
\Pr_{a,b}[\lambda_{ab}>1/2]< 2\mathbb{E}_{a,b}[\lambda_{ab}]< O(\eps).
$$
Thus, we have:
$$
\Pr_{a,b}\left[ f(a)=f(b)+\sum_i g_i(b,a_i)  \right] > 1-O(\eps).
$$
Then, by the probabilistic method there exists $\beta$ such that 
$$
\Pr_a\left[ f(a)=f(\beta)+\sum_i g_i(\beta,a_i) \right]>1-O(\eps).
$$
That is, $f$ is $O(\eps)$-close to the direct sum $a\mapsto f(\beta)+\sum_i g_i(\beta,a_i)$.

\end{proof}

==> notes/affinity-old.tex <==
\section{Trying to get direct sumness from being affine on subcubes}
\todo{not working yet}
\begin{claim}
 $k_a(b)$ is $24\eps_a$-close to a constant $k(a)$.
\end{claim}
\begin{proof}
 Sample $b^{(0)}, b^{(1)},b^{(2)},b^{(3)},b^{(4)}$ as follows:
 Sample $b^{(0)}, b^{(4)}$ uniformly randomly. 
 Then, let $(\pi_1,\pi_2,\pi_3, \pi_4)$ be a random partition of $[d]$ into four equally sized  parts. 
 For $i=1,2,3$, set $b^{(i)}_j$ equal to $b^{(i-1)}_j$ if $j\notin \pi_i$ and $b^{(4)}_j$ if $j\in \pi_i$.
 
 Observe that (marginally), for each $i\in \{0,1,2,3\}$, the points $b^{(i)},b^{(i+1)}$ are uniformly random, conditioned on the fact that they agree in $3d/4$  coordinates.
 Thus, $k_a(b^{(i)}) = k_a(b^{(i+1)})$ with probability at least $1-6\eps_a$ for each $i\in \{0,1,2,3\}$.
 Taking a union bound we find that $k_a(b^{(0)})=k_a(b^{(1)})$ with probability at least $1-24\eps_a$.
 Thus, there is some value $k(a)$ such that $\Pr_{b}[k_a(b)-k(a)]>1-24\eps_a$.
\end{proof}
 

\begin{claim}
 There exist functions $\psi_1,\dots,\psi_d$ such that 
 $$
 \Pr_{a,b}[g_i(a,b_i)=\psi_i(a_i,b_i) \;\forall i]>1-O(\eps).
 $$
\end{claim}
 \todo{ is this claim actually true?}

Combining Claim 3 with Lemma 1 (via a union bound) we have:
$$
\Pr_{a,b,x} \left[ f(S_x(a,b))=k(a)+\sum_i \psi_i(a_i, b_i)x_i \right] > 1-O(\eps).
$$
This concludes the proof of Lemma 2 $\square$.

---


\begin{lemma}
 $$
 \Pr_{a,b,x}\left[ f(S_x(a,b))=\sum_i \phi_i(a_i)\overline{x_i}+\phi_i(b_i)x_i\right]> 1-O(\eps).
 $$

\end{lemma}
Now, we recall from earlier that 
$$
\Pr_{a,b}\left[ k(a)=\sum_i g_i(b,a_i)+k(b) \right]>1-O(\eps).
$$
Thus, there exists $\beta$ such that 
$$
\Pr_a\left[ k(a)=\sum_i g_i(\beta,a_i)+k(\beta) \right]>1-O(\eps).
$$
Let $\Phi(a) = \sum_i g_i(\beta,a_i)+k(\beta) = \sum_i \phi_i(a_i)$. 
We have shown that $k(a)$ is $O(\eps)$ close to the direct sum $\Phi(a)$.
Taking another union bound we have 
$$
\Pr_{a,b,x}\left[ f(S_x(a,b))=\sum_i \phi_i(a_i) + \sum_i \psi_i(a_i,b_i)x_i \right] > 1-O(\eps).
$$

 \begin{claim}
 $$
 \Pr_{a,b}[\psi_i(a_i,b_i)=\phi_i(a_i)+\phi_i(b_i) \; \forall i] > 1-O(\eps).
 $$
 \end{claim}
 \begin{proof}
 Use the fact that $S_x(a,b)=S_{\bar{x}}(b,a)$ 
 \todo{ spell this out. I feel confident that it will work though}
 \end{proof}

Applying Claim 4 and another union bound we have, 
$$
\Pr_{a,b,x}\left[ f(S_x(a,b))=\sum_i \phi_i(a_i)\overline{x_i}+\phi_i(b_i)x_i\right]> 1-O(\eps).
$$

Now, note that if $a,x,b$ are sampled randomly then $S_x(a,b)$ is a uniformly random point in the domain. 
Hence, 
$$
\Pr_z \left[ f(z)=\sum_i \phi_i(z_i) \right]>1-O(\eps).
$$

==> notes/broken.tex <==
\section{Broken}
\begin{definition}
  Test 8 is the following test: (todo come up with catchier name)
Sample $a,b,x$. Return YES iff
\[ f(a)+f(b)+f(a_xb) + f(b_x a)=0. \] 
\end{definition}

\begin{theorem}
Let $f:\F_2^d \to \F_2$.
If $f$ is linear then $f$ passes Test 8 with probability $1$. 
If $f$  passes Test 8 with probability $1-\eps$ then  $f$ is $O(\eps)$-close to
a linear function.
\end{theorem}
\begin{proof}

First, consider what this means about $f$ restricted to the subcube $C_{a,b}$.
Here we can write it like
\[ f(0)+f(1)+f(x)+f(x+1) = 0. \] 

Case 1: $f(0)+f(1)=0$.
Then we have
 \[ \Pr_x[f(x)+f(x+1)=0] > 1-\eps. \] 
\todo{Wait no, this is not how probabilities work.}
Switching to multiplicative notation for convenience (i.e., $\F_2 \to
\set{-1,1}$) we can write this like:
\[ \E_x f(x)f(-x) > 1-2\eps. \] 


A basic fourier analysis fact is that $\E_x f(x)g(x) = \sum
\widehat{f}(S)\widehat{g}(S)$. 
Thus, we get 
\[ \sum_{|S| \text{ even}} \widehat{f}(S)^2 - \sum_{|S|\text{ odd}}
\widehat{f}(S)^2 > 1-2\eps. \] 
So this means 
\[ \sum_{|S|\text{ even}} \widehat{f}(S)^2 > 1-\eps. \] 
Put another way, $f$ is $\eps$-close to being even.

Case 2: $f(0)+f(1)=1$. Sorry I omit it for now. But probably it just says that
all the fourier mass is on odd-sized characters.


okok. So at this point we have shown that restricted to a random $C_{a,b}$ we
are close to even / odd. 
Now we claim that the only way this can happen is if we are linear. 

Suppose that you can partition the characters into two groups $A,B\subseteq[n]$
such that 
 \[ \sum_{S\in A} \widehat{f}(S)^2 > 100\eps, \sum_{S\in B} \widehat{f}(S)^2 >
100\eps. \] 
Then, I claim that with probability at least $1/1000$ when you do the
restriction thing $f$ won't be super close to an even or odd function.

You can see this by seeing that a decent fraction of the $A$ characters become
odd-sized with decent probabilty and a decent fraction of the $B$ characters become
even-sized with decent probabilty.

Anyways either Alek or Edward should write this up nicer at some point and think
about annoying edge cases like the empty character.

But the vibes are that we will conclude that $f$ has a character on which it has
weight like $1-100\eps$ or something, and that's just saying that $f$ is close
to linear. 

\end{proof}


\begin{proof}
\todo{I had some approach that I thought would be better. Here are some ideas for it.}
\todo{actually I'm not sure what I'm hoping to gain from this approach.}
Suppose you sample $f(x|0), f(y|0), f(y|a), f(x|a)$ where $x,y,a$ are random.
It's quite unlikely that both $f(x|0), f(y|0)$ are corrupted. Then by summing we will distinguish between $f(x|0),f(y|0)$ both being uncorrupted and exactly one being corrupted. 
This should be boostable.

Sample $x^{(1)}, \ldots, x^{(T)}\in [n]^{d-1}$.
With probability $1-\binom{T}{2}\eps$ I can get accurate values for $\sum_{i=1}^{d-1} L_i(x_i^{(j)})+L_i(x_i^{(k)})$ for all $k,j$.
Once I have done this, I can build a graph on the $x^{(j)}$'s where I put an edge between two dudes if they are either both good or both bad. 
Here good and bad are defined by whether $f(x^{(j)}|0) = L(x^{(j)}|0).$

This will split the graph into two components, and I think it is extremely likely that the larger component is the good one. 
I haven't computed how likely yet. 

Anyways, you could probably use this to recover the value of $f(0)$.
Maybe there's also a more efficient way to do this though. 

Yeah I think we get exponential Chernoff stuff here. 
\end{proof}

Here's a more promising indication that we can do better. 
\begin{proposition}
    Suppose $f: [2]^d \to \F_2$ is $\eps$ close to a direct sum $L=\oplus_i L_i$. 
    Suppose $\eps< 1/8.$
    Then we can determine the value of $L(b)$ for arbitrary $b$ with good probability and not too many queries. 
\end{proposition}
\begin{proof}
    You can \emph{independently} test for each coordinate whether that coordinate is ``influential'' or not. 
    In total this requires $O(d\log d)$ queries to succeed with constant probability. In $O(d\log(d/\delta))$ queries we can succeed with probability $1-\delta$.
\end{proof}


> [!tip] Claim 2
> $k_a(b)$ is $24\eps_a$-close to a constant $k(a)$.
> 
> **proof of claim:**\
> Sample $b^{(0)}, b^{(1)},b^{(2)},b^{(3)},b^{(4)}$ as follows:
> Sample $b^{(0)}, b^{(4)}$ uniformly randomly. 
> Then, let $(\pi_1,\pi_2,\pi_3, \pi_4)$ be a random partition of $[d]$ into four equally sized  parts. 
> For $i=1,2,3$, set $b^{(i)}_j$ equal to $b^{(i-1)}_j$ if $j\notin \pi_i$ and $b^{(4)}_j$ if $j\in \pi_i$.
> 
> Observe that (marginally), for each $i\in \{0,1,2,3\}$, the points $b^{(i)},b^{(i+1)}$ are uniformly random, conditioned on the fact that they agree in $3d/4$  coordinates.
> Thus, $k_a(b^{(i)}) = k_a(b^{(i+1)})$ with probability at least $1-6\eps_a$ for each $i\in \{0,1,2,3\}$.
> Taking a union bound we find that $k_a(b^{(0)})=k_a(b^{(1)})$ with probability at least $1-24\eps_a$.
> Thus, there is some value $k(a)$ such that $\Pr_{b}[k_a(b)-k(a)]>1-24\eps_a$.



> [!tip] Claim 3
> There exist functions $\psi_1,\dots,\psi_d$ such that 
> $$
> \Pr_{a,b}[g_i(a,b_i)=\psi_i(a_i,b_i) \;\forall i]>1-O(\eps).
> $$
> 
> **Proof of claim:**
> #todo is this claim actually true?

Combining Claim 3 with Lemma 1 (via a union bound) we have:
$$
\Pr_{a,b,x} \left[ f(S_x(a,b))=k(a)+\sum_i \psi_i(a_i, b_i)x_i \right] > 1-O(\eps).
$$
This concludes the proof of Lemma 2 $\square$.

---


> [!tip] Lemma 3
> $$
> \Pr_{a,b,x}\left[ f(S_x(a,b))=\sum_i \phi_i(a_i)\overline{x_i}+\phi_i(b_i)x_i\right]> 1-O(\eps).
> $$

**Proof of Lemma 3**
Now, we recall from earlier that 
$$
\Pr_{a,b}\left[ k(a)=\sum_i g_i(b,a_i)+k(b) \right]>1-O(\eps).
$$
Thus, there exists $\beta$ such that 
$$
\Pr_a\left[ k(a)=\sum_i g_i(\beta,a_i)+k(\beta) \right]>1-O(\eps).
$$
Let $\Phi(a) = \sum_i g_i(\beta,a_i)+k(\beta) = \sum_i \phi_i(a_i)$. 
We have shown that $k(a)$ is $O(\eps)$ close to the direct sum $\Phi(a)$.
Taking another union bound we have 
$$
\Pr_{a,b,x}\left[ f(S_x(a,b))=\sum_i \phi_i(a_i) + \sum_i \psi_i(a_i,b_i)x_i \right] > 1-O(\eps).
$$

> [!tip] Claim 4
> $$
> \Pr_{a,b}[\psi_i(a_i,b_i)=\phi_i(a_i)+\phi_i(b_i) \; \forall i] > 1-O(\eps).
> $$
> **Proof of Claim**:
> Use the fact that $S_x(a,b)=S_{\bar{x}}(b,a)$ 
> #todo spell this out. I feel confident that it will work though

Applying Claim 4 and another union bound we have, 
$$
\Pr_{a,b,x}\left[ f(S_x(a,b))=\sum_i \phi_i(a_i)\overline{x_i}+\phi_i(b_i)x_i\right]> 1-O(\eps).
$$

Now, note that if $a,x,b$ are sampled randomly then $S_x(a,b)$ is a uniformly random point in the domain. 
Hence, 
$$
\Pr_z \left[ f(z)=\sum_i \phi_i(z_i) \right]>1-O(\eps).
$$




==> notes/error-correction-old.tex <==
\begin{proposition}
Fix $\eps>0, n\in \N$, and $d$ odd. Suppose $\min(n\eps + d^2/n, n\eps d) <
1/4$, and that $f:[n]^d\to \F_2$ is $\eps$-close to the direct sum $L=\sum_i L_i$. 
Then, the Shapka test recovers the correct value for $L(b)$, for arbitrary $b$,
with probability at least $3/4$.
\end{proposition}
\begin{proof}

Fix functions $f,L$ as in the proposition statement, and suppose we want to
obtain the value of $L$ at a point $b$.
We say that a query $f(x)$ \defn{succeeds} if $f(x)=L(x)$.
Let $\eps_i = \Pr_x[f(x)=L(x)\mid x_i = b_i]$.
By the principle of inclusion-exclusion we have 
$$\Pr_x[f(x)\neq L(x)]\ge \sum_i \Pr[f(x)\neq L(x) \land x_i =b_i] - \sum_{i\neq j}\Pr[f(x)\neq L(x)\land x_i=b_i \land x_j=b_j].$$
Thus, $$\eps \ge \sum \eps_i / n - (d/n)^2.$$ 
This implies that $$\sum \eps_i \le n\eps+d^2/n.$$
The following bound is also evident: for each $i$,
$$\eps=\Pr[f(x)\neq L(x)]\ge \Pr[f(x)\neq L(x)\land x_i = b_i]=\eps_i/n.$$
Thus,
$$\sum \eps_i \le n\eps d \le 1/4.$$
Thus, the Shapka test produces the correct value with probability at least $3/4$.
\end{proof}

==> semi-old-stuff/affinity-new.tex <==
\section{Affine on Subcube Test}
In \cite{di19} Dinur and Golubev define the \defn{Square in Cube} test\footnote{They actually consider a slightly more general setting, where the domain is $[n_1]\times \cdots\times[n_d]$. For simplicity, we restrict our attention to the case $n_i = n_j$ for all $i,j$.}.
\begin{test}[Square in Cube]\label{def:squarecube}
Sample random $a,b\in [n]^d$ and $x,y\in \mathbb{F}_2^{d}$ and test:
$$ 
f(S_0(a,b)) + f(S_x(a,b))+ f(S_y(a,b))+f(S_{x+y}(a,b))=0.
$$ 
\end{test}
They claim that if $f$ passes the Square in Cube test with probability $\eps$,
then $f$ is $O(\eps)$-close to a direct sum. However, their is a problem with
their analysis. They establish that $f$ is \emph{locally} a direct sum (this is
essentially \cref{cor:dp} in our presentation), but they do not show that these
local direct sums agree. In this section we provide a corrected analysis of this
test, and a more general class of tests. The Square in Cube test can be viewed
as performing the BLR test on a random subcube. We show that in fact testing for
affinity on a random subcube, with \emph{any}  affinity tester, also works as a
direct sum test.
Combined with our results in \cref{sec:diamond} this allows us to show that the
Diamond test is a direct sum test. The flexibility of being able to use any
affinity tester also enables us to obtain a direct sum test with additional
properties, e.g., erasure resiliency \cite{erasure}. 

\begin{test}[Affine on Subcube test]
Pick random $a,b\in [n]^d$ and run an affinity test on $x\mapsto f(S_x(a,b))$.
\end{test}

\begin{proposition}
If $f$ is $\eps$-close to a direct sum then $f$ passes the affine on subcube test with probability at least $1-4\eps$.
\end{proposition}
\begin{proof}
By a union bound with probability at least $1-4\eps$ our queries are all made to locations where $f$ agrees with the closest direct sum to $f$. 
The restriction of a direct sum to a subcube is affine, so direct sums pass the test with probability $1$. The conclusion follows.
\end{proof}
Now, we show the test is sound: if it passes with good probability then $f$ is close to a direct sum.
\begin{theorem}\label{thm:subcube-affinity}
Fix $n,d\in \N$.
Suppose $f:[n]^d\to \F_2$ passes an affinity test on a random subcube with probability $\eps$. Then $f$ is $Cn\eps$ close to a direct sum for some constant $C$ depending on the affinity test, but not on $d,n$.
\end{theorem}
\begin{proof}
Fix $f:[n]^d\to \F_2$  which passes the Affine on Subcube test with probability $1-\eps$ for some fixed affinity test.
For each $a,b$ define $f_{ab}$ to be the function $x\mapsto f(S_x(a,b))$ (the restriction of $f$ to a subcube), and let $\eps_{ab}$ be the probability that $f_{ab}$ fails the affinity test. We have $\E[\eps_{ab}] = \E[\eps_a] = \eps.$
Because $f_{ab}$ passes the affinity test with probability $1-\eps_{ab}$, there is vector $F_a(b) \in \F_2^d$ and constant $k_{a}(b)$ such that
$$ \Pr_x[f_{ab}(x)=\ang{F_a(b), x}+k_{a}(b)]>1-O(\eps_{ab}), $$
where $\ang{v,w} = \sum_i v_i w_i$.

\begin{lemma}\label{lem:fabdirectprod}
$b\mapsto F_a(b)$ is $O(\eps_a)$-close to a direct product $(g_{1}^a(b_1),\dots,g_d^a(b_d))$, and $b\mapsto k_a(b)$ is $O(\eps_a)$-close to a constant $k(a)$.
\end{lemma}

\begin{proof}
Define distribution $b'\sim D_{b}, b'\in [n]^d$ as follows: 
\begin{quote}
Sample $b'$ uniformly randomly, conditional on having $b_i'= b_i$ hold for exactly $3d/4$ of $i\in [d]$. 
\end{quote}
Define distribution $x\sim X_{bb'},x\in \mathbb{F}_2^d$ as follows:
\begin{quote}
$x_i=0$ for all $i\in \Delta(b,b')$,
and, if $b_i=b_i'$ then $x_i=1$ with probability $2/3$ and $0$ else.
\end{quote}
Observe: For any $x_{0}\in \mathbb{F}_2^d$, $\Pr_{b,b'\sim D_{b},x\sim X_{bb'}}[x=x_{0}]=1/2^d$. 
That is, $x$ is uniformly distributed, and pairwise independent of $b,b'$, although of course the triple $(x,b,b')$ is not uniformly random on $\F_2^d \times [n]^d\times [n]^d$. 
By construction, $S_x(a,b) = S_x(a,b')$ (whenever $b_i,b_i'$ differ, we choose $a_i$).
Then, by a union bound (and averaging away $b$ in our earlier expression) we have that 
$$
\Pr_{b,b'\sim D_{b},x\sim X_{bb'}} [\ang{F_a(b),x}+k_a(b) =f(a_xb) = f(a_xb') = \ang{F_a(b'), x}+k_a(b')] > 1-2\eps_{a}.
$$
Let 
$$
\delta_{abb'} =  \Pr_{x\sim X_{bb'}} [\ang{F_a(b)\oplus F_a(b'), x} \neq k_a(b)+k_a(b')].
$$
Let $\overline{\Delta}(b,b')$ denote the set of indices $i$ where $b_i=b_i'$. For vector $x\in \mathbb{F}_2^d$, and set $S\subseteq [d]$, let $x\mid_S$ denote the restriction of $x$ to coordinates $S$. Then,

\begin{claim}
If $\delta_{abb'}<1/3$ then $F_a(b)\mid_{\overline{\Delta}(b,b')}= F_a(b')\mid_{\overline{\Delta}(b,b')}$ and $k_a(b)=k_a(b')$.
\end{claim}
\begin{proof}
Assume for sake of contradiction that there exists  $i\in \Delta(F_a(b), F_a(b')) \cap \overline{\Delta}(b,b')$.
Sampling $x\sim X_{bb'}$ we have a $1/3$ chance of $x_i$ being $0$ and a $2/3$ chance of $x_i$ being $1$, independent of the values of $x_j$ for $j\neq i$.
But then $\ang{F_a(b)\oplus F_a(b'), x}$ doesn't take on any value in $\mathbb{F}_2$ with probability greater than $2/3$, contradicting $\delta_{abb'}<1/3$.
Thus, $\Delta(F_a(b), F_a(b')) \cap \overline{\Delta}(b,b') = \varnothing$.

We have shown that if $\delta_{abb'}<1/3$ then for any $x\sim X_{bb'}$ we have $\ang{F_a(b)\oplus F_a(b'),x} = 0$.
Thus, if $\delta_{abb'}<1/3$ we must have $k_a(b)=k_a(b')$.
\end{proof}

Now, by Markov's Inequality we have that 
$$
\Pr_{b,b'\sim D_{b}}[\delta_{abb'}>1/3] \le 3\mathbb{E}_{b,b'}[\delta_{abb'}] < 6\eps_a.
$$
From this we conclude
$$
\Pr_{b,b'\sim D_{b}} [F_a(b)\mid_{\overline{\Delta}(b,b')}= F_a(b')\mid_{\overline{\Delta}(b,b')}] > 1-6\eps_a.
$$
\todo{oops need to state DP theorem}
\todo{also, note that the DP theorem can be stated with the approx size 1/4 thing not exactly 1/4. maybe have to cite Dinur for this.}

By  \cref{fact:directproduct} we conclude that $F_a(b)$ is $O(\eps_a)$-close to a direct product $(g_1(a,b_1),\dots,g_d(a,b_d))$. 

\begin{claim}
 $k_a(b)$ is $24\eps_a$-close to a constant $k(a)$.
\end{claim}
\begin{proof}
 Sample $b^{(0)}, b^{(1)},b^{(2)},b^{(3)},b^{(4)}$ as follows:
 Sample $b^{(0)}, b^{(4)}$ uniformly randomly. 
 Then, let $(\pi_1,\pi_2,\pi_3, \pi_4)$ be a random partition of $[d]$ into four equally sized  parts. 
 For $i=1,2,3$, set $b^{(i)}_j$ equal to $b^{(i-1)}_j$ if $j\notin \pi_i$ and $b^{(4)}_j$ if $j\in \pi_i$.
 
 Observe that (marginally), for each $i\in \{0,1,2,3\}$, the points $b^{(i)},b^{(i+1)}$ are uniformly random, conditioned on the fact that they agree in $3d/4$  coordinates.
 Thus, $k_a(b^{(i)}) = k_a(b^{(i+1)})$ with probability at least $1-6\eps_a$ for each $i\in \{0,1,2,3\}$.
 Taking a union bound we find that $k_a(b^{(0)})=k_a(b^{(1)})$ with probability at least $1-24\eps_a$.
 Thus, there is some value $k(a)$ such that $\Pr_{b}[k_a(b)-k(a)]>1-24\eps_a$.
\end{proof}
\end{proof}

Let $T_{1/2}(a)$ denote the distribution on $[n]^d$ obtained by sampling random $b,x$ and outputting $a_xb$.
Using \cref{lem:fabdirectprod} we obtain:
\begin{corollary}\label{cor:dp}
For all $a\in [n]^d$, there exists a direct product $(g^a_1,\ldots, g^a_d):\F_2^d\to \F_2^d$ and value $\eps_a$ such that
$$ \Pr_{b\sim T_{1/2}(a)}[f(b) = \sum_i g_i^a(b_i)] > 1-\eps_a, $$ 
where the $\eps_a$ satisfy $\E_a \eps_a \le O(\eps)$.
\end{corollary}
\begin{proof}
We know that 
$$ \Pr_x[f(a_xb)=\ang{F_{a}(b),x}+k_{a}(b)]>1-O(\eps_{ab}). $$
\cref{lem:fabdirectprod} tells us that $F_a(b)$ is close to a direct product $(g^a_1,\ldots, g^a_d)$ and $k_a(b)$ is close to a constant $k^a$.
Thus, by a union bound
$$  \Pr_{x,b} \left[ f(a_xb) = k^a + \sum_i g_i^a(b_i)x_i \right] > 1-O(\eps_a).  $$
Then, by changing some variable names we can obtain the corollary.
\end{proof}

The following lemma will be useful.

\begin{lemma}\label{lem:dps_independence}
Let $\mathcal{D}$ be some probability distribution over $[n]^d$
where each coordinate is independent, and for each $i\in [d],x\in [n]$ we have $\Pr_{c\sim \mathcal{D}}[c_i=x] \ge .1/n$.
Suppose that direct sums $F,F': [n]^d\to \F_2$ satisfy
$$ \Pr_{c\sim \mathcal{D}}[F'(c) = F(c)] > 1-.1/n. $$
Then, $F'=F$.
\end{lemma}
\begin{proof}
First, observe that for each $i$ the difference $F_i'-F_i$ must be consistent or
there is no hope $F,F'$ agreeing with sufficiently good probability.
Thus, there exist constants $c_i$ such that 
$$F_i(x) = c_i + F_i(x),$$
for all $i,x$.
But then we must have
$$\Pr_{c\sim \mathcal{D}}\left[\sum c_i = 0\right]> 1-.1/n,$$
implying that $\sum c_i = 0$, whereby we have
$F' = F$.
\end{proof}

\begin{lemma}\label{lem:gaeqgb}
$$ \Pr_{a,b}[g^a = g^b]> 1-O(n\eps). $$ 
\end{lemma}

\begin{proof}
Let $B_{1/4}(a)$ be the set of points that disagree with $a$ on
at most $1/4$ of their coordinates.
Fix $a,b\in B_{1/4}(a)$.
Let $r\ge 3/4$ be the fraction of coordinates on which $a_i,b_i$ agree.
Define distribution $c\sim \mathcal{D}$ as follows:
\begin{itemize}
\item If $a_i=b_i$, then $c_i = a_i$ with probability $(1/2-1/(2n))/r+1/n$ and
sample it uniformly randomly from $[n]\setminus \set{a_i}$ otherwise.
\item If $a_i\neq b_i$, then sample $c_i$ uniformly randomly.
\end{itemize}
We now make some observations about this distribution.
First, observe that 
\[ \Pr[c_i = a_i \mid a_i = b_i] = (1/2-1/(2n))/r+1/n  \le 2/3. \] 
The fact that this probability is less than $1$ makes our distribution well
defined, while the fact that this probability is bounded away from $1$ will be
important later.
Second, observe that at each coordinate $i$, 
$$\Pr[a_i = c_i] = \Pr[b_i = c_i] = r\cdot \left( (1/2-1/(2n))/r+1/n \right) +
(1-r)/n  = \frac{1}{2} + \frac{1}{2n}.$$ 
That is, $c$ has the same distribution as $T_{1/2}(a)$ (if we
don't look at $b$) and as $T_{1/2}(b)$ (if we don't look at $a$).
Define $g^a(x) = \sum_i g^a_i(x)$, where $g^a$ is the function given in \cref{cor:dp}.
Define 
$$\delta_a = \Pr_{b\sim T_{1/2}(a)}[f(b)\neq g^a(b)].$$
By \cref{cor:dp} we have $\delta_a \le O(\eps_a)$.
Thus, by \cref{cor:dp} we have:
$$ \Pr_{c\sim \mathcal{D}}[f(c)\neq g^a(c) \bigvee f(c)\neq g^b(c)]\le \delta_a+\delta_b). $$
By a union bound this means:
$$ \Pr_{c\sim \mathcal{D}}[g^a(c) = g^b(c)]\ge 1-(\delta_a+\delta_b). $$
Now, because $g^a,g^b$ are direct sums, by \cref{lem:dps_independence} we have
that if $\delta_a+\delta_b < .1/n$, then 
$$ g^a = g^b. $$ 
Of course, by Markov's inequality we have:
$$ \Pr_{a,b\in B_{1/4}(a)}[\delta_a+\delta_b<.1/n]>1-O(n\eps). $$ 
Thus, 
$$ \Pr_{a,b\in B_{1/4}(a)}[g^a=g^b] > 1-O(n\eps). $$ 
Finally, taking a sequence $a_1,a_2,a_3,a_4,a_5$ where $a_i,a_{i+1}$ are each
$3/4$ correlated but  $a_1,a_5$ are just random independent points, and using a
union bound, we have that:
$$ \Pr_{a,b}[g^a = g^b] > 1-O(n\eps). $$ 
\end{proof}

Now we finish proving the theorem.
Combining \cref{cor:dp} and \cref{lem:gaeqgb} we have:
$$ \Pr_{a,b,c\sim T_{1/2}(b)} [g^a \neq g^c  \bigvee  g^c(b)\neq f(b)] \le O(n\eps). $$ 
Thus, 
$$ \Pr_{a,b}[g^a(b) = f(b)] > 1-O(n\eps).$$ 
Then, by the probabilistic method we can choose $a$ such that $f$ is $O(n\eps)$ close to the direct sum $g^a$.

\end{proof}


==> semi-old-stuff/diamond-weak.tex <==
Thus, we will focus our attention on showing that the Diamond test is an
affinity tester for $f: \F_2^{d}\to \F_2$.
We believe that the Diamond test may also be of independent interest as, to the
best of the authors' knowledge, it is a novel linearity test. 

\subsection{A Weak Analysis of the Diamond Test}

In this section we show that the diamond test is at least somewhat good at rejecting functions which are far from affine: if $f$ is $\eps$ far from affine, the Diamond test rejects with probability $\Omega(\eps/d^{1.1})$.
The dependence on $d$ is undesirable, and in future sections we will discuss attempts at achieving stronger quantitative results.

\todo{more description text here}

\begin{lemma}\label{lem:bday}
    Suppose $X\subset \F_2^d$  has $|X|\ge .99 |\F_2^d|$, and let $d$ be at
    least a sufficiently large constant.
    Then, there exists a subset $B\subset X$, with $|B|= \ceil{1.02\log_2 d}$, 
    such that for any $i\in [d]$ $B$ contains both a vector $x$ with $x_i = 1$
    and a vector $x'$ with $x_i'=0$.
\end{lemma}
\begin{proof}
By the probabilistic method it is sufficient to demonstrate that a randomly chosen $B\subset X$ has the desired property with non-zero probability. 
Fix some coordinate $i\in [d]$.
The probability that $B$ only contains vectors of a single parity at coordinate $i$ is at most
$$2(100/198)^{\ceil{1.02\log_2 d}}< 1/(2d).$$
By a union bound the probability that there is any coordinate where $B$ lacks vectors of both parities at the coordinate is at most $1/2$.
\end{proof}

\begin{lemma}\label{lem:diamond}
There exist $b,c$ such that 
$$
\Pr_{a,x}\left[f(a)=f(a_xb)f(c_xa)f(c_xb)\right]>1-2\eps.
$$
\end{lemma}
\begin{proof}
We perform the following two tests:
$$
f((a_xd)_xb)f(b_x(a_xd)) = f(a_xd)f(b)
$$
$$
f(b_x(c_xd))f((c_xd)_xb) = f(c_xd)f(b).
$$
It may be more clear to think of these like this:
$$
f(a_xb)f(b_xd) = f(a_xd)f(b)
$$
$$
f(b_xd)f(c_xb) = f(c_xd)f(b).
$$
If $a,b,c,d,x$ are sampled uniformly randomly then these are both uniformly random tests, although they are correlated. 
By a union bound, the tests simultaneously pass with probability $1-2\eps$.
Thus, we have 
$$\Pr_{a,b,c,d,x}\left[f(a_xb)f(a_xd)=f(c_xd)f(c_xb)\right]>1-2\eps.$$
Renaming variables again we get:
$$
\Pr_{a,c,d,x}\left[f(a) = f(a_xd)f(c_xd)f(c_xa)\right]>1-2\eps.
$$
By the probabilistic method we can choose $c,d$ such that 
$$\Pr_{a,x}\left[f(a) = f(a_xd)f(c_xd)f(c_xa)\right]>1-2\eps.$$
\end{proof}

\begin{lemma}
\label{lem:refine}
Suppose there is a partition $I=(I_1,\ldots, I_k)$  of $[d]$ and there are functions $g_1,\ldots, g_k$ with $g_i: \F_2^{I_i}\to \pm 1$, and there is $\xi$ such that:
$$
\Pr_a \left[f(a) = \prod_i g_i(a_{I_i})\right]>1-\xi.
$$
Suppose further that there exists a partition $J_0\sqcup J_1=[d]$ and functions $h_0:\F_2^{J_0}\to \pm 1,h_1:[2]^{J_1}\to\F_2$ and $\eps$  such that 
$$\Pr_a \left[f(a) = \prod_j h_j(a_{J_j})\right]>1-\eps.$$
Then there exist functions $\ell_{i,j}:[2]^{I_i\cap J_j}\to \F_2$ such that 
$$\Pr_a\left[  f(a) = \prod_{i,j}\ell_{i,j}(x_{I_i\cap J_j}) \right] > 1-2(\eps+\xi)-\eps.$$
\end{lemma}
\begin{proof}
By a union bound, with probability $\eps+\xi$ over choice of $a$ we get:
$$
\prod_i g_i(a_{I_i}) = \prod_j h_j(a_{J_j}).
$$
For each $j$, by the probabilistic method, there exists $a_{\overline{J_j}}$ such that 
$$\Pr_{a_{J_j}} \left[h_j(a_{J_j}) = h_{j+1}(a_{\overline{J_{j}}}) 
\prod_i g_i(a_{I_i})
\right] > 1-(\eps+\xi).$$
We can interpret this as the existence of the $\ell_{i,j}:[2]^{I_i\cap J_j}\to \F_2$ described in the lemma statement.
Finally, by another union bound we have 
$$\Pr_a\left[  f(a) = \prod_{i,j}\ell_{i,j}(x_{I_i\cap J_j}) \right] > 1-2(\eps+\xi)-\eps.$$
\end{proof}

Now we combine the three lemmas to prove the following:
\begin{theorem}
    If $f:\F_2^d \to \pm 1$ passes the diamond test with probability $\eps$ then is is at least $O(d^{1.02}\eps)$ close to linear. 
\end{theorem}
\begin{proof}
Call $x$ \defn{good} if 
$$\Pr_a[f(a) = f(a_xb)f(c_xa)f(c_xb)]>1-100\eps.$$
By \cref{lem:diamond} we have:
$$\E_x[\Pr_a[f(a) \neq f(a_xb)f(c_xa)f(c_xb)]]<2\eps.$$
Thus, by Markov's Inequality, at least $99$\% of $x$ are good.
Now, by \cref{lem:bday} we can find good $x^{(1)},\ldots, x^{(\ceil{1.02\log d})}$ such that for each $i\in [d], b\in \F_2$ there is some vector $x^{(j)}$ with $x^{(j)}_i=b$.
Now we repeatedly apply \cref{lem:refine} and XXX.

\todo{finish some details}
\end{proof}
\input{strong_diamond}

To prove that the Diamond test is an affinity tester, it remains to show:
\begin{conjecture}\label{conj:rejrej}
Suppose $f$ is $.01$-far from affine.
Then, the Diamond test rejects $f$ with probability at least $.00001.$
\end{conjecture}

\begin{remark}
One piece of evidence for this is that the diamond test rejects the majority function with constant probability.

You can see this as follows:
With constant probability, $wt(a)$ is 1 SD to the left of $n/2$ and $wt(b)$ is 10 SD's to the right of $n/2$. 
In this case, it's pretty likely that both $wt(a_xb)$ and $wt(b_xa)$ are to the right of $n/2$. So the diamond test will reject.
\end{remark}

\begin{remark}
The small $\eps$ analysis should still go through just fine if we do 
$$(a,b)\sim \mathsf{eq}_{3/4}$$
Where this distribution is just ``make them agree on $3/4$ of the coordinates'', instead of the default $\mathsf{eq}_{1/2}$.
Nothing special about $3/4$ either. 
\end{remark}


\subsection{Derivative Approach for Analyzing Diamond Test in Large Influence Case}
In this subsection we give another potential approach to analyzing the Diamond test, albiet in a special case.

\begin{proposition}
Let $f$ be a function which is $\eps^{1/4}$-far from affine, and which has a cooridinate with influence at least $\eps^{1/4}$.
Then, the diamond test rejects $f$ with probability at least $\Omega(\eps)$.
\end{proposition}
\begin{proof}

Assume for sake of contradiction that $f: \pmo^n  \to  \pmo$ satisfies the following conditions:
\begin{enumerate}
    \item The diamond test rejects $f$ with probability less than $\eps$,
    \item $f$ is $\eps^{1/4}$-far from linear,
    \item $f$ has a coordinate with influence at least $\eps^{1/4}$.
\end{enumerate}
Then, 
$$ \E_R[\text{dist}(Rf, \eo)]=\eps. $$
So, by Markov
$$ \Pr_R[\text{dist}(Rf, \eo)<10\sqrt{ \eps }]>1-\sqrt{ \eps }/10. $$
Let $i$ be the maximum influence coordinate of $f$. Then, 
$$ f(x_i,x_{-i}) = g(x_{-i})x_i+h(x_{-i}), $$
where $||g||^{2}>\eps^{1/4}, ||h||^2 > \eps^{1/4}$.
Now, the hypercube is broken up into two regions: one where $g=0, |h|=1$ and one where $h=0, |g|=1$.

At this point we'd like to show:
\begin{equation}\label{eq:bothbig}
\Pr_R[||Rg||^{2}>40\sqrt{ \eps }  \land ||Rh||^{2}> 40\sqrt{ \eps }]>\sqrt{ \eps }.
\end{equation}
This would contradict our earlier statement about how the restriction is extremely likely to be very close to $\eo$. I'll spell this out below.
It seems plausible that the extremal case (the setup that would the probability \cref{eq:bothbig} smallest) is when $h$ is supported on a subcube. And in this extremal case we seem to do quite well. 

Specifically the lemma we're missing is something like this:
\todo{don't include this subsection unless you can prove this conjecture, probably}
\begin{conjecture}
Let $A,B$ be a partition of the subcube, where $\mu(A),\mu(B)>\eps^{1/4}$.
Then, if we do a random restriction where we choose $1/2$ of the coordinates randomly, and restrict these chosen coordinates randomly to $\pm 1$, there is at least a $\sqrt{\eps}$ chance that we end up with $\mu_R(A),\mu_R(B) > 40\sqrt{\eps}$.
\end{conjecture}
\begin{remark}
    This conjecture is true in the case that $A$ is supported on a subcube. Which feels like the worst case. Here's the analysis on a subcube.

\begin{framed}
The claim that I'll make is basically something like this:
$$
\Pr_R[{\mu_R(A)<\eps}] < 1-\mu(A)^{\log_2(4/3)}
$$
although not quite this. 
The argument for this was just "how do I make $\mu_R(A)$"  be very likely to be small? put it on a subcube. so it isn't quite what i need but is close 

Then I'll say:
$$
\Pr_R[\mu_R(A)<\eps \bigvee \mu_R(B)<\eps ]\le 1-\mu(A)^{.7} + 1-\mu(B)^.7 < 1-\eps^.3
$$
because $\mu(A)+\mu(B)=1$, and because exponents play nice I guess.
And thus, 
$$\Pr_R[\mu_R(A)]>\eps \bigwedge \mu_R(B)>\eps] >\eps^{.3},$$
which is like exactly what I needed. 
\end{framed}
\end{remark}

Now, I show that if the event in \cref{eq:bothbig} happens, then with probability $\Omega(1)$ the restriction of the final variable makes us far from $\eo$.
Suppose that we did the restriction, and we got some decomposition like 
$$ Rf(y, z) = z(a(x)+b(x))+c(x)+d(x),$$
where  $||a+b||^{2} > 40\sqrt{\eps},||c+d||^{2} > 40\sqrt{\eps}$, and where $a,c$ are the Even parts and $b,d$ are the Odd parts.
Let's try to make it so that all three possible things --- not touching $z$, fixing $z$ to $+1$, and fixing $z$ to $-1$ --- result in the final restriction being $10\sqrt{\eps}$-close to $\eo$ (spoiler: this will be impossible).

First, we must ensure that if we don't restrict $z$ then the function is close to $\eo$. To ensure this we must have that one of $||a||^{2}+||c||^{2}, ||b||^{2}+||d||^{2}$ is large and the other is tiny. 
Without loss of generality, assume
$$||a||^{2}+||c||^{2}<10\sqrt{\eps}, ||b||^{2}+||d||^{2}>1-10\sqrt{\eps}.$$
Recalling that $||a+b||^2,||c+d||^2$ are both at least $20\sqrt{\eps}$, we then have (by the triangle inequality)
$$||b||^2, ||d||^2> 30\sqrt{\eps}.$$
Now, consider what happens when we restrict $z$, for instance to $+1$.
In order for the restriction to be $10\sqrt{\eps}$-close to $\eo$ we must have one of $||a+d||^2, ||c+b||^2$ larger than $1-10\sqrt{\eps}$ and the other smaller than $10\sqrt{\eps}$.
However, by the triangle inequality we have:
$$||a+d||^2 \ge ||d||^2-||a||^2> 20\sqrt{\eps},$$
and 
$$||c+b||^2 \ge ||b||^2-||c||^2> 20\sqrt{\eps}.$$
Thus, it is impossible for this restriction to have the desired property.

\end{proof}


\section{More Thoughts on the Diamond Test}

\begin{proposition}
If $f$ is a non-linear $O(1)$-Junta, then the test rejects with decent probability. 
\end{proposition}
\begin{proof}
This is because we know the test rejects with probability at least $\eps/d$ or something.
\end{proof}

\begin{lemma}
AFSoC: $\mathsf{dist}(f, \mathsf{AFFINE}) = \mu(1f) >1/64$, BUT $\Pr[f(a)+f(b)=f(a_xb)+f(b_xa)]>.99999$.
Then: 
(1) 
$$
\Phi(1f) \approx \mu \cdot \Pr_{a,b\in 1f, x}[a_xb \in \overline{1f}] + (1-\mu)/2.
$$
and (2)
$$
\Phi(1f) \leq 1/2 + (\mu/2)\cdot \Pr_{a,b\in 1f,x}[\{ a_xb, b_xa \}\subset \overline{1f} ].
$$

\todo{actually, it doesn't seem like this is saying anything more useful than}
$$\Phi(1f)\le (1+\mu)/2.$$
\todo{So this is definitely not going to be sufficient for $\mu>1/3$}
\end{lemma}
\begin{proof}
   It's pretty standard. 
   The interesting thing is you can move in two different ways and you get these two different inequalities.
\end{proof}

\begin{remark}
Let $f$ be distance $\mu(1f)>1/64$ from affine.
AFSoC diamond test passes with probability $.9999$.
Then, 
$$\Pr_{a\in S, b\in \bar{S}}[a_xb \in S] \approx 1/2$$
$$Pr_{a\in S, b\in S}[axb \in S] + Pr_{a\in \bar{S}, b\in \bar{S}}[axb \in S] \cdot (1/\mu-1)^2 \approx 1.$$
\end{remark}

\newcommand{\affine}{\mathsf{affine}}
\begin{remark}
    One interesting function is the majority function.
    The majority function has $\Phi(1f) = 1/3$.
    It also has $\dist(f, \affine) \approx 1/2$.
    Finally, it has $\Pr_{a,b\in 1f,x}[a_xb\in \overline{1f}] = 0$.
    So, for the marjotiy function
    $$1/3 = \Phi(1f) \ge (1-\mu)/2 = 1/4. $$
\end{remark}

\begin{remark}
If $\mu(1f)\le 1/16$ for instance, then the trivial bound of $\Phi(1f)\ge 1-\mu ^{1/3}$ already serves to give a contradiction.
Some non-trivial understandings of the probabilities in these expressions could boost us to something like $1/8$ or $1/4$ respectively.
But to actually win, we probably want better expansion bounds for functions that are far from being $O(1)$-juntas.
\end{remark}

\subsection{More Thoughts}
\newcommand{\heart}{\heartsuit}
\newcommand{\stab}{\mathsf{stab}_{1/2}}
Edward's pattern idea:

Sample pattern $P$ with $1/2$ ?'s $1/4$ $+$'s and $1/4$ $-$'s.
We say $a\heart b$ if $(a\in S \land b\in S) \lor (a \in \bar{S} \land b \in \bar{S}).$
Call a pattern \defn{good} if $\Pr_{(a,b)\sim P}[a \heart b] \in [0,0.01]\cup[.99,1]$.
We can show that the probability that a random pattern is good is at least $.9999$ (under the assumption test that diamond test is bad at rejecting $f$, even though $\mu(f)>1/64$).


\subsection{Noise Stability}
Another observation: 
might be interesting to record for each $a$ the value of 
$$ \Pr_{b\sim T_{1/2}(a)}[b\heart  a] $$
Define:
$$\stab(f) = 1-2\Pr_{x, y\sim T_{1/2}(x)}[f(x)\neq f(y)] = 2\Pr_{x,y\sim T_{1/2}(x)}[x\heart y]-1.$$
Fact: $$ \stab(f) = \sum  2^{-|S|} \hat{f}(S)^{2}. $$

\begin{framed}
\noindent{\color{red}The key problem in all of this is that we don't know how to use the condition of being far from linear!!}
\end{framed}


\subsection{Diamond Test for $\eps=0$}

\begin{proposition}
    If the diamond test passes with probability $1$, then $f$ is affine.
\end{proposition}
\begin{proof}
$$
\forall x,a: f(a) = f(0)+f(a_x 0) + f(0_x a).
$$
So, we can take $f(a)$ and decompose it into $\sum_i a_i\cdot (f(e_i)+f(0))$, making $f$ affine.
\end{proof}

\begin{remark}
   One consequence of this is that the diamond test works well on functions which are close to small Juntas. 
\end{remark}


==> semi-old-stuff/diamond.tex <==
\section{The Diamond Test}\label{sec:diamond}
In \cite{di19}, Dinur and Golubev propose analyzing the following test, which we call the
\defn{Diamond in Cube} test as an open question:
\begin{test}[Diamond in Cube]
Sample random $a,b\in [n]^d,x\in \F_2^d$. Accept iff
$$f(a)+f(b)=f(\phi_x(a,b))+f(\phi_x(b,a)).$$
\end{test}
We note that, to the best of the authors' knowledge, this test was not
previously understood in the setting $n=2$. That is, an analysis of the Diamond
in Cube test for the case $n=2$ gives a novel affinity tester for functions
$f:\F_2^d\to \F_2$. This is in contrast to Dinur and Golubev's Square in Cube
test for direct sum, which reduces to the BLR \cite{BLR} tester in the case of
$n=2$.
In this section we will analyze the Diamond in Cube test in the case of $n=2$. 
In \cref{sec:subcube} we will give a general result, that will imply as a corollary
that the Diamond in Cube test is a direct sum tester for $n> 2$ as well (with
some caveats, see \cref{sec:subcube} for details.

Our analysis of the $n=2$ case is intriguing. 
We now give a rough sketch of the ideas used in the analysis.
First, we generalize to a ``4-function'' version of the test, which is more amenable to induction.
Then, we use hypercontractivity (\cite{hyper1},\cite{hyper2}) to prove
\cref{thm:dichotomy}, which establishes a dichotomy for 4-tuples of functions
that pass the test with probability $1-\eps$: either the functions are all
$O(\eps)$-close to affine, or one of them is $\Omega(1)$-far from affine.
Then, we relate the probability of the test passing on functions $(f,g,h,k)$ to
the probability of the test passing on restrictions of $(f,g,h,k)$, allowing us to
induct on the dimension of $f$. Crucially, the dichotomy theorem allows us to
avoid our closeness factor deteriorating at each step of the induction, which
would result in a dependence on the dimension in our result.
This dichotomy based approach is inspired by work of \cite{david2015direct}, but
the details of establishing the dichotomy and performing the induction are quite
different.
We will also derive an interesting Fourier analytic fact as a consequence of our
analysis of the Diamond in Cube test.

For the $n=2$ case, we will analyze a slightly more general test, which we call
the $\rho$-Diamond test; this will be important for extending to the case of
$n>2$. To define this test, we extend the definition of  the noise operator to allow negative correlations. 
Specifically, for $x\in \F_2^d$ and $p\in [0,1]$, we define the distribution
$y\sim \T_{-p}$ as follows: for each $i\in [d]$ independently, set $y_i=x_i+1$ with probability $p$ and sample $y_i$ randomly otherwise. Then, the $\rho$-Diamond test is defined as follows:
\begin{test}[$\rho$-Diamond test]
Sample $a,x\sim \F_2^d,b\sim \T_{\rho}(a)$. Accept iff 
$$f(a)+f(b) = f(\phi_x(a,b)) + f(\phi_x(b,a)).$$
\end{test}
When $\rho$ is clear from context we abbreviate $\rho$-Diamond test to
\defn{Diamond test}. For simplicity, we encourage the reader to think of the
case $\rho=0$ (i.e., $a,b$ are uncorrelated) when reading the proof.
As a preliminary sanity check, and as the base case for our induction, we observe:
\begin{lemma}\label{lem:rhobasecase}
Fix $\rho\in (-1,1)$.
$f$ is affine if and only if $f$ passes the $\rho$-Diamond test with probability $1$.
\end{lemma}
\begin{proof}
If $f$ is a direct sum $f(x) = \sum_i L_i(x_i)$, then 
$$f(a)+f(b)  = \sum_i (L_i(a_i)+L_i(b_i)) = f(\phi_x(a,b)) + f(\phi_x(b,a)).$$
Now, suppose $f$ passes the Diamond test with probability $1$. Then, for all $x,a\in \F_2^d$ we have
\begin{equation}\label{eq:breakitup}
f(a) = f(0)+f(\phi_x(0,a)) + f(\phi_x(a,0)),
\end{equation}
where $0$ denotes the zero vector. Let $e_i\in \F_2^d$ denote a vector which is
$0$ at all coordinates except coordinate $i$.
Then, repeated application of \cref{eq:breakitup} lets us decompose  $f(a)$ as 
$$f(a) = f(0)+\sum_{i=1}^d \left(f(a_i e_{i})+f(0)\right),$$
indicating that $f$ is affine.
\end{proof}
The completeness of our test is trivial:
\begin{proposition}
Fix $\rho\in (-1,1)$. If $f:\F_2^{d}\to \F_2$ is $\eps$-close to affine, the $\rho$-Diamond test
passes with probability at least $1-4\eps$.
\end{proposition}
\begin{proof}
Let $g$ be affine with $\dist(f,g)\le \eps$. By a union bound, $f$ and $g$ agree
on all $4$  points queried by the test (because each query is marginally
uniformly distributed), in which case the Diamond  test accepts.
by \cref{lem:rhobasecase}.
\end{proof}

Now we turn to showing that the Diamond test is sound.
\input{smallepsilon}
\input{weak-diamond}
\input{strong_diamond}
\input{fourierfact}



==> semi-old-stuff/old-junta-degree-stuff.tex <==
\section{Junta-Degree $k$ Testing}

In this section, we consider the generalization of direct sum testing to
\textbf{junta-degree $k$} testing, i.e., testing whether $f$ is the sum of
functions which only look at $k$ bits of the input at a time (direct sum being
the case $k=1$). Using a similar technique to the Affine on Subcube test, we
show how to test whether a function $f: S_1\times \cdots \times S_d \to \F_q$,
for any $2$ element sets $S_1,\ldots, S_d\subseteq \F_q$, is a restriction of a
degree $k$ polynomial over $\F_q$ to an asymmetric grid. Such a test was already
given in by Bafna, Srinivasan, Sudan \cite{srinivasan2018local}; our test
improves the query complexity of this previous work. This complements recent
work in \cite{amireddy2023low} by Amireddy, Srinivasan and Sudan which shows
that this is impossible if the sets $S_i$ are instead allowed to be of size $3$.

Formally, we say that a function $f:[n]^d\to \F_q$ is Junta-degree $k$ if there exist
functions $g_S: [n]^{S}\to \F_q$ for each $S\in \binom{[d]}{k}$ such that 
\[ f(x) = \sum_{S} g_S(x_S). \] 
An important ingredient in our analysis will be a generalization of the
\cite{dinur2014direct}'s direct product test (\cref{test:dp}) to a \defn{$k$-direct product} test.
We say that $F:[n]^d \to \F_2^{\binom{[n]}{k}}$ is a $k$-direct product if there
are functions $\setof{G_S}{S\in \binom{[n]}{k}}$ so that for each $S\in
\binom{[n]}{k},x\in [n]^d$, we have $F_S(x)=G_S(x_S)$.
We conjecture:
\begin{conjecture}\label{conj:highdimdp}
Fix integers $n,d,k$.
Let $F: [n]^d \to \F_2^{\binom{[d]}{\le k}}$, satisfy the following agreement condition:
$$\Pr_{b,b'\sim T_{3/4}(b)} \left[F_{S}(b) = F_{S}(b') \quad \forall S\in \binom{[d]}{\le k} \mid b_S = b'_S\right] > 1-\eps.$$ 
Then, there are functions $\setof{g_S:\F_2^{S}\to \F_2}{S\in \binom{[d]}{\le k}}$ such that 
$$\Pr_{b}\left[F_S(b) = g_S(b_S) \quad\forall S\in \binom{[d]}{\le k}\right] > 1-O_k(\eps).$$
\end{conjecture}
For $n>2$ we do not know of a proof of this conjecture in the literature,
although we believe that techniques in the literature could be adapted to prove this result.
For $n=2$ Dinur et al. \cite{dinur2017agreement} have already analyzed this test:
\begin{fact}[Higher Dimensional Agreement Theorem \cite{dinur2017agreement}]\label{fact:multidp}
\cref{conj:highdimdp} is true for $n=2$.
\todo{Look into what the constant is...}
\end{fact}
Thus, we will be content to analyze our test for the case $n=2$ which is
interesting \todo{cite some literature}.
We remark that we believe that resolving \cref{conj:highdimdp} is the main
missing ingredient required to obtain Junta-Degree $k$ testing for $n>2$.

% \todo{
% \begin{fact}[Higher Dimensional Agreement Theorem \cite{dinur2017agreement}]\label{fact:multidp}
% Suppose you have a collection of local functions
% $\setof{f_S : \binom{S}{k} \to \Sigma}{S\in \binom{[d]}{d/2}}$ satisfying 
% \[ \Pr_{(T, S_1, S_2)\sim \mu_n(d/4,d/2)} [f_{S_1}\mid_T = f_{S_2}\mid_T] \le \eps. \] 
% Where this $\mu_n(d/4,d/2)$ thing means, choose $S_1,S_2$ of size $d/2$ with
% intersection $S_1\cap S_2 = T$ of size $d/4$, and $v_n(k)$ is just a random
% $k$-element set.

% Then, the majority decoded function $G: \binom{[d]}{k} \to \Sigma$ satisfies 
% \[ \Pr_{S \sim v_n(k)}[f_S \neq G\mid_S] \le C_k \eps. \] 

% And supposedly the $C_k$ dependence is not so good. 
% \end{fact}
% }


Using \cref{fact:multidp}, and generalizing the ideas from
\cref{thm:subcube-affinity} we will prove the following theorem.
\begin{theorem}
Fix $d,k\in \N$, and fix $n=2$.
Suppose the expected distance to degree $k$ functions of the restriction of
$f:[n]^d\to \F_2$ to a random subcube is $\eps$. Then $f$ is $C_k\eps$-close to
a direct sum for some constant $C_k$ depending on the degree $k$ test, but not
on $n,d$.
\end{theorem}
\begin{proof}

For each $a,b$, let $F^{ab}$ denote the closest degree $k$ function to $x\mapsto f(a_xb)$. Define
\begin{equation}\label{epsab:final}
\eps_{ab} = \Pr_{x}[f(a_xb) \neq F^{ab}(x)].
\end{equation}
We have $\E_{ab}[ \eps_{ab} ] = \eps.$

\begin{lemma}\label{lem:closemultidp}
$b\mapsto F^{ab}$ is $O_k(\eps_a)$-close to a $k$-direct product.
\end{lemma}
\begin{proof}
Define distribution $b'\sim D_{b}, b'\in [n]^d$ as follows: 
\begin{quote}
Sample $b'$ uniformly randomly, conditional on having $b_i'= b_i$ hold for exactly $3d/4$ of $i\in [d]$. 
\end{quote}
Define distribution $x\sim X_{bb'},x\in \mathbb{F}_2^d$ as follows:
\begin{quote}
$x_i=0$ for all $i\in \Delta(b,b')$,
and, if $b_i=b_i'$ then $x_i=1$ with probability $2/3$ and $0$ else.
\end{quote}
Observe: For any $x_{0}\in \mathbb{F}_2^d$, $\Pr_{b,b'\sim D_{b},x\sim X_{bb'}}[x=x_{0}]=1/2^d$. 
That is, $x$ is uniformly distributed, and pairwise independent of $b,b'$, although of course the triple $(x,b,b')$ is not uniformly random on $\F_2^d \times [n]^d\times [n]^d$. 
By construction, $S_x(a,b) = S_x(a,b')$ (whenever $b_i,b_i'$ differ, we choose $a_i$).
Then, by a union bound (and averaging away $b$ in our earlier expression) we have that 
$$
\Pr_{b,b'\sim D_{b},x\sim X_{bb'}} [F^{ab}(x) =f(a_xb) = f(a_xb') = F^{ab'}(x)] > 1-2\eps_{a}.
$$
Let 
$$
\delta_{abb'} =  \Pr_{x\sim X_{bb'}} [F^{ab}(x)\neq F^{ab'}(x)].
$$
It will be convenient to use the decomposition 
\[F^{ab}(x) = \sum_{S \in \binom{[d]}{\le k}} F^{ab}_S \prod_{i\in S}x_i. \] 
Define $$A_{bb'} = \setof{S\in \binom{[d]}{\le k}}{b_i = b_i' \forall i\in S}.$$
\begin{claim}
If $\delta_{abb'} < 1/3^{k}$, then for all $S\in A_{bb'}$, $F^{ab}_S = F^{ab'}_S$.
\end{claim}
\begin{proof}
This is a simple consequence of the fact that in the $2/3$-biased hypercube, all
non-zero degree-$k$ polynomials are distance at least $1/3^{k}$ from zero.
For completeness we prove this fact in \cref{fact:distancetozero}
\end{proof}
\begin{fact}\label{fact:distancetozero}
In the $2/3$-biased hypercube, all non-zero degree-$k$ polynomials are distance
at least $1/3^{k}$ from zero.
\todo{state this a bit more generally}
\end{fact}
\begin{proof}
We induct on the degree $k$.
The base case is trivial. Assume the claim for degree $k-1$. Given a
degree-$k$ polynomial $f(x)$, choose some variable $z$ that has a non-zero
coefficient and write: 
\[ f(y,z) = z g(y) + h(y), \] 
where $g$ a non-zero degree $k-1$ polynomial.
Let 
\[ \psi = \Pr_{y\sim \mu_{2/3}^{\otimes d-1}} [g(y)\neq h(y)]. \] 
Because $g$ is a degree $k-1$ polynomial, 
\[ \Pr_{y\sim \mu_{2/3}^{\otimes d-1}} [g(y)\neq 0] \ge 3^{1-k}. \] 
We can bound the chance of $f$ being zero as follows:
\begin{align*}
\Pr_{y,z\sim \mu_{2/3}^{\otimes d}} [f(y,z)\neq 0] 
&\ge \frac{2}{3} \psi + \frac{1}{3}  \Pr_{y\sim \mu_{2/3}^{\otimes d-1}} [h(y)\neq 0]  \\
&\ge  \frac{2}{3}\psi + \frac{1}{3} \cdot \max(0, 3^{1-k} - \psi)\\
&\ge  3^{-k}.
\end{align*}
\end{proof}

Now, by Markov's Inequality we have that 
$$
\Pr_{b,b'\sim D_{b}}[\delta_{abb'}>3^{-k}] \le
3^{k}\mathbb{E}_{b,b'}[\delta_{abb'}] < O(3^{k}\eps_a).
$$
From this we conclude
$$
\Pr_{b,b'\sim D_{b}} [ \forall S\in A_{bb'}, F^{ab}_S = F^{ab'}_S] \ge 1-O(3^{k}\eps_a).
$$

Then, applying \cref{fact:multidp} finishes the proof of the lemma.

\end{proof}

It is helpful to restate this as follows:
\begin{corollary}\label{cor:kdirectsum}
For each $a$, there exists $G^a = \setof{G^a_S:[n]^S\to \F_2}{S\in \binom{[d]}{\le k}}$
such that 
$$\Pr_{b\sim T_{1/2}(a)}\left[f(b) = \sum_S G^a_S(b_S) \right] > 1-O_k(\eps_a).$$
\end{corollary}
\begin{proof}
Performing a union bound on \cref{epsab:final} and \cref{lem:closemultidp} we have
$$\Pr_{a,x,b}\left[f(a_xb) = \sum_S G^a_S(b_S) \prod_{i\in S} x_i \right] > 1-O_k(\eps_a),$$
where $G^a_S$ is the closest $k$-direct product to $b\mapsto F^{ab}$.
Then, we define
$$\widetilde{G^a}_S((a_xb)_S) = G^a_S(b_S) \prod_{i\in S} x_i.$$
This is well defined because if $\prod_{i\in S} x_i = 0$, then we give the value
$0$, and if $x_i = 1$ for all $i\in S$ then $(a_xb)_S = b_S$.
Then, 
$$\Pr_{b\sim T_{1/2}(a)}\left[f(b) = \sum_S \widetilde{G^a_S}(b_S) \right] > 1-O_k(\eps_a).$$
\end{proof}
In \cref{cor:kdirectsum} we have shown that \emph{locally} our function $f$ is close to junta-degree $k$.
To finish, we will show that these local junta-degree $k$ functions agree.
First, we need the following lemma about junta-degree $k$ functions.

\begin{lemma}\label{lem:multidp_indep}
Let $\mathcal{D}$ be some probability distribution over $[n]^d$ where each
coordinate is independent and for each $i\in [d], x\in [n]$ we have 
$\Pr_{y\sim \mathcal{D}}[y_i = x]  > .1/n.$
Suppose that junta-degree $k$ functions $F,F': [n]^{d}\to \F_2$ satisfy
$$ \Pr_{y\sim \mathcal{D}}[F'(y) = F(y)] > 1-(.1/n)^k.$$
Then, $F'=F$.
\end{lemma}
\begin{proof}
Recall that we are assuming $n=2$, so junta-degree $k$ is the same thing as being a degree $k$ polynomial. Thus,  \cref{fact:distancetozero} implies the lemma. 
\end{proof}

\begin{lemma}
$$ \Pr_{a,b}[G^a = G^b]> 1-O(n\eps). $$ 
\end{lemma}
\begin{proof}
Let $B_{1/4}(a)$ be the set of points that disagree with $a$ on
at most $1/4$ of their coordinates.
Fix $a,b\in B_{1/4}(a)$.
Let $r\ge 3/4$ be the fraction of coordinates on which $a_i,b_i$ agree.
Define distribution $y\sim \mathcal{D}$ as follows:
\begin{itemize}
\item If $a_i=b_i$, then $y_i = a_i$ with probability $(1/2-1/(2n))/r+1/n$ and
sample it uniformly randomly from $[n]\setminus \set{a_i}$ otherwise.
\item If $a_i\neq b_i$, then sample $y_i$ uniformly randomly.
\end{itemize}
We now make some observations about this distribution.
First, observe that 
\[ \Pr[y_i = a_i \mid a_i = b_i] = (1/2-1/(2n))/r+1/n  \le 2/3. \] 
The fact that this probability is less than $1$ makes our distribution well
defined, while the fact that this probability is bounded away from $1$ will be
important later.
Second, observe that at each coordinate $i$, 
$$\Pr[a_i = y_i] = \Pr[b_i = y_i] = r\cdot \left( (1/2-1/(2n))/r+1/n \right) +
(1-r)/n  = \frac{1}{2} + \frac{1}{2n}.$$ 
That is, $y$ has the same distribution as $T_{1/2}(a)$ (if we
don't look at $b$) and as $T_{1/2}(b)$ (if we don't look at $a$).
Define $g^a(x) = \sum_S G^a_S(x_S)$, where $G^a$ is the $k$-direct product given in \cref{cor:kdirectsum}.
Define 
$$\delta_a = \Pr_{b\sim T_{1/2}(a)}[g^a(b)\neq f(b)].$$
By \cref{cor:kdirectsum} we have $\delta_a \le O_k(\eps_a)$.
Then,
$$ \Pr_{y\sim \mathcal{D}}[f(y)\neq g^a(y) \bigvee f(y)\neq g^b(y)]\le \delta_a+\delta_b. $$
By a union bound this means:
$$ \Pr_{c\sim \mathcal{D}}[g^a(c) = g^b(c)]\ge 1-(\delta_a+\delta_b). $$
Now, because $g^a,g^b$ are direct sums, by \cref{lem:multidp_indep} we have
that if $\eps_a+\eps_b < (.1/n)^k$, then 
$$ g^a = g^b. $$ 
Of course, by Markov's inequality we have:
$$ \Pr_{a,b\in B_{1/4}(a)}[\eps_a+\eps_b<(.1/n)^k]>1-O_k((10n)^k\eps). $$ 
Thus, 
$$ \Pr_{a,b\in B_{1/4}(a)}[g^a=g^b] > 1-O_k((10n)^k\eps). $$ 
Finally, taking a sequence $a_1,a_2,a_3,a_4,a_5$ where $a_i,a_{i+1}$ are each
$3/4$ correlated but  $a_1,a_5$ are just random independent points, and using a
union bound, we have that:
$$ \Pr_{a,b}[g^a = g^b] > 1-O_k((10n)^k\eps). $$ 
\end{proof}

Now we finish proving the theorem.
$$ \Pr_{a,b,c\sim T_{1/2}(b)} [g^a \neq g^c  \bigvee  g^c(b)\neq f(b)] \le O((10n)^k\eps). $$ 
Thus, 
$$ \Pr_{a,b}[g^a(b) = f(b)] > 1-O((10n)^k\eps).$$ 
Then, by the probabilistic method we can choose $a$ such that $f$ is
$O((10n)^k\eps)$ close to the junta-degree $k$ function $g^a$.
    
\end{proof}


==> semi-old-stuff/pbiased_diamond.tex <==
\newcommand{\DP}{\mathcal{D}_p}
\section{The Diamond Test}\label{sec:diamond}
We restate the Diamond in the Cube test, initially proposed by Dinur and Golubev in \cite{di19} (recall from \cref{sec:prelims} that $\phi_x$ is the interpolation function)
\begin{test}[Diamond in Cube]\label{test:diamondcube}
Sample random $a,b\in [n]^d,x\in \F_2^d$. Accept iff
$$f(a)+f(b)=f(\phi_x(a,b))+f(\phi_x(b,a)).$$
\end{test}
% We note that, to the best of the authors' knowledge, this test was not
% previously understood in the setting $n=2$. That is, an analysis of the Diamond
% in Cube test for the case $n=2$ gives a novel affinity tester for functions
% $f:\F_2^d\to \F_2$. This is in contrast to Dinur and Golubev's Square in Cube
% test for direct sum, which reduces to the BLR \cite{BLR} tester in the case of
% $n=2$.
We will show that \cref{test:diamondcube} is a valid tester for direct sum. As is usual in property testing, 
it is straightforward to verify that any direct sum passes with probability $1$ and so completeness holds. The remainder of the section is focused on showing soundness via the following theorem.

\begin{theorem} \label{thm:diamond_cube_soundness}
    Suppose $f: [n]^d \xrightarrow[]{} \F_2$ passes the Diamond in the Cube Test with probability $1-\epsilon$. Then, $f$ is ... close to a direct sum.
\end{theorem}

Our proof proceeds as follows. We begin by considering a $p$-biased version of the Diamond in the Cube test in the $n = 2$, or hypercube, case --- which we simply call the Diamond test. After establishing soundness in this setting, we then boost to the general $n$ setting by viewing the overall Diamond in the Cube test as choosing a random, induced, hypercube in $[n]^d$, and then performing the $p$-biased Diamond test inside of this hypercube for an appropriately chosen $p$. Altogether, this will give us many local direct sums that nearly agree with $f$ on many induced hypercubes inside of $[n]^d$. To conclude we use a direct product testing result of \cite{dinur2014direct} to show that there is a global direct sum consistent with many of the local direct sums. This global direct sum is also close to $f$ and so we are done. 

The $p$-biased hypercube case is analyzed in \cref{sec: n=2 case}, the application of direct product testing is done in \cref{sec:subcube}, and we conclude the proof of soundness by combining the two parts in \cref{sec:conclude soundness diamond}.

\subsection{Step 1: The $p$-biased $n = 2$ Case} \label{sec: n=2 case}
In this section we consider a $p$-biased version of the Diamond in the Cube Test in the $n = 2$ case. Here it will be convenient for us to view the domain as $\F_2^d$ instead of $[2]^d$ and refer to direct sums over $\F_2^d$ as affine functions. We also refer to \cref{test:diamondcube} simply as the Diamond test for the $n = 2$ case. The $p$-biased generalization of the Diamond test that we consider is the following:
\begin{test}\label{test:diamond test}[$p$-Biased Diamond]
Sample $a,x\sim \F_2^{d}$, and $b\sim \T_p(a)$. Accept if and only if
$$f(a)+f(b)=f(\phi_x(a,b))+f(\phi_x(b,a)).$$
\end{test}
We will often refer to the $p$-Biased Diamond test as simply the Diamond test when $p$ is
clear from context. We encourage the reader to focus on the case of $p=0$ (i.e.,
the Diamond test). We will usually fix $p\in (-1,1)$ before specifying $n,d$,
meaning $|p|$ is thought of as bounded away from $1$ by some constant; the dependence
of our results on this constant will be hidden by our asymptotic notation.

The goal of this section is to show that \cref{test:diamond test} is a valid affinity tester  over $\F_2^d$. As a warm up, let us consider what happens when the test passes with probability $1$. This case will be useful to us later on and also establishes the diamond test's completeness.

\begin{lemma}\label{lem:basecase}
Fix $p\in (-1,1)$. The function
$f: \F_2^d \xrightarrow[]{} \F$ is affine if and only if $f$ passes the $p$-Biased Diamond test with probability $1$.
\end{lemma}
\begin{proof}
If $f$ is affine then we can write $f(x) = \sum_i L_i(x_i)$. It follows that for any $a,b \in \F_2^d$,
$$f(a)+f(b)  = \sum_i (L_i(a_i)+L_i(b_i)) = f(\phi_x(a,b)) + f(\phi_x(b,a)).$$
For the other direction, suppose $f$ passes the Diamond test with probability $1$. Then, for all $x,a\in \F_2^d$ we have
\begin{equation}\label{eq:breakitup}
f(a) = f(0)+f(\phi_x(0,a)) + f(\phi_x(a,0)),
\end{equation}
where $0$ denotes the zero vector. Let $e_i\in \F_2^d$ denote a vector which is
$0$ at all coordinates except coordinate $i$.
Then, repeated application of \cref{eq:breakitup} lets us decompose  $f(a)$ as 
$$f(a) = f(0)+\sum_{i=1}^d \left(f(a_i e_{i})+f(0)\right),$$
indicating that $f$ is affine.
\end{proof}
As a simple corollary of \cref{lem:basecase} we have:
\begin{corollary}
If $f$ is $\eps$-close to affine, then $f$ passes the Diamond test with probability at least $1-4\eps$.
\end{corollary}
\begin{proof}
Let $g$ be affine with $\dist(f,g)\le \eps$. By a union bound, $f$ and $g$ agree
on all $4$  points queried by the test (because each query is marginally
uniformly distributed), in which case the Diamond  test accepts.
by \cref{lem:basecase}.
\end{proof}

With completeness done, the remainder of this section is focused on showing soundness. Specifically, we show the following theorem.
\begin{theorem}\label{cor:1fun}
Fix $p\in (-1,1)$.
If $f$ passes the $p$-Biased Diamond test with probability $1-\eps$, then $f$ is
$O_p(\eps)$-close to affine. 
\end{theorem}

Our analysis of the $n=2$ case is both technically interesting and provides a new result on affinity testing over $\F_2^d$. We start with a rough sketch of the ideas used in the analysis.
First, we will generalize to a ``4-function'' version of the test, which is more amenable to induction.
Then, we use hypercontractivity (\cite{hyper1},\cite{hyper2}) to prove
\cref{thm:dichotomy}, which establishes a dichotomy for 4-tuples of functions
that pass the test with probability $1-\eps$: either the functions are all
$O(\eps)$-close to affine, or one of them is $\Omega(1)$-far from affine.
Next, we will relate the pass probability of $(f,g,h,k)$ to the pass probability of restricted versions $(f,g,h,k)$ with one coordinate fixed. This reduces allows us to go down one dimension and apply induction.
Crucially, the dichotomy theorem allows us to
avoid our closeness factor deteriorating at each step of the induction, which
would result in a dependence on the dimension in our result.
This dichotomy based approach is inspired by the work of \cite{optimalreedmuller, david2015direct}, but
the details of establishing the dichotomy and performing the induction are quite
different.

\subsubsection{The Four Function Version}

In order to facilitate our inductive approach, it will be more convenient to work with a four function version of the diamond test. The one function version of the diamond test can be considered a special case where $f = g= h = k$.
\begin{test}[$p$-Biased 4-Function Diamond]
Sample $a,x\sim \F_2^d, b\sim \T_p(a)$, and accept if and only if
\[ f(a)+k(b) = g(\phi_x(a,b)) + h(\phi_x(b,a)). \] 
\end{test}
The following lemma characterizes what happens when four functions pass with probability $1$. It will be used later to establish the base case (in constant dimensions) of our inductive analysis.
\begin{lemma}\label{lem:4basecase}
Fix $p\in (-1,1)$.
Suppose $(f,g,h,k)$ passes the $p$-Biased 4-function Diamond test with probability $1$.
Then, there is a linear function $L$ such that $f,g,h,k$ are all equal to either $L$ or $L+1$.
\end{lemma}
\begin{proof}
If $(f,g,h,k)$ passes the 4-function Diamond test with probability $1$ then for all $a,x,b$ we have:
\[ f(a)+g(\phi_x(a,b))+h(\phi_x(b,a))+k(b)=0=f(b)+g(\phi_{x+\one}(b,a))+h(\phi_{x+\one}(a,b))+k(a). \] 
Using \cref{fact:fliperoo} to simplify we get that for all $a,b$,
\[ f(a)+k(a)=f(b)+k(b). \] 
Again using the fact that $(f,g,h,k)$ passes the test with probability $1$ we have that for all $a,x,b$:
\[ f(a)+g(\phi_x(a,b))+h(\phi_x(b,a))+k(b)=0=f(a)+g(\phi_{x+\one}(a,b))+h(\phi_{x+\one}(b,a))+k(b). \] 
By \cref{fact:fliperoo} this implies
\[ g(\phi_x(a,b))+g(\phi_{x}(b,a)) = h(\phi_x(a,b))+h(\phi_{x}(b,a)). \] 
Letting $c=\phi_x(a,b),d=\phi_{x}(b,a)$, and noting that $c,d$ can be
arbitrary (unrelated) elements of  $\F_2^{d}$, we have that for all $c,d$.
\[ g(c)+g(d)  = h(c)+h(d).\] 
Combining our observations so far we conclude that there exist constants
$\alpha,\beta$ such that for all $a\in \F_2^{d}$ we have
\[ f(a)=k(a) +\alpha, \quad g(a) = h(a)+\beta.\] 
Thus, for all $a,b$ we have
\[ f(a)+f(b)=g(\phi_x(a,b))+g(\phi_x(b,a))+\alpha+\beta. \] 
Taking $x=0$ we conclude
\[ f(a)+f(b) = g(a)+g(b)+\alpha+\beta. \] 
Thus, there exists $\gamma$ such that  for  all $a$ we have
\[ f(a)=g(a)+\gamma.\] 
In summary, we have shown that for all $a,b,x$, we have
\[ f(a)+f(b)=f(\phi_x(a,b))+f(\phi_x(b,a))+\alpha+\beta. \] 
Setting $x=0$ again shows that $\alpha+\beta = 0$.
Thus, we have that $f$ passes the (1-function) Diamond test with probability $1$.
By \cref{lem:basecase} this implies that $f$ is affine.
Finally, recall that we have shown in the course of our proof that $g,h,k$ all
differ from $f$ by a constant. This concludes the proof.
\end{proof}

\subsubsection{A Dichotomy for Functions Passing the Diamond Test}
We are now prepared to show \cref{thm:dichotomy}, which states
that if the 4-function Diamond test accepts $(f,g,h,k)$ with probability exactly
$1-\eps$ then $f$ is either $O(\eps)$-close to affine, or $\Omega(1)$-far from affine. To this end, we first establish two lemmas which will useful in
the proof. Let $\DP$ denote the following distribution on $(\F_2^{d})^3$:
sample a triple $(a,x,b)$ by first taking $a,x\sim \F_2^{d}$ and then taking
$b\sim\T_p(a)$.

\begin{lemma}\label{lem:fghconst}
Fix $p\in (-1,1)$.
Fix $d\in \N$ and functions $f,g,h:\F_2^{d}\to \F_2$.
Suppose $f,g,h$ have
\[ \Pr_{(a,x,b)\sim\DP}[f(a)+g(\phi_x(a,b))+h(\phi_x(b,a))=1]<\eps. \] 
Then, $f,g,h$ are $3\eps$-close to constants.
\end{lemma}
\begin{proof}
Fix $f,g,h$ as in the theorem. 
Performing a union bound and using \cref{fact:fliperoo} we have
\[ \Pr_{(a,x,b)\sim\DP}[f(a)+g(\phi_x(a,b))+h(\phi_x(b,a))=f(b)+g(\phi_x(a,b))+h(\phi_x(b,a))] >  1-2\eps.\] 
Thus, $f$ is $2\eps$-close to a constant $\alpha$.
Then, by a union bound we have
\[ \Pr_{(a,x,b)\sim\DP}[g(\phi_x(a,b))+h(\phi_x(b,a))=\alpha+1]>1-3\eps. \] 
Of course, the distribution of $(\phi_x(a,b),\phi_x(b,a))$ is the same as the
distribution of $(a,b)$.
Thus, we have
\[ \Pr_{a\sim\F_2^{d},b\sim\T_p(a)}[g(a)+h(b)= \alpha+1]>1-3\eps. \] 
By the probabilistic method this implies that $g,h$ are each $3\eps$-close to
constants.
\end{proof}

We will also need the following lemma, which is a slightly modified version of the classic \defn{small set expansion} property of the noisy hypercube (see \cite{od21}).
\begin{lemma}\label{lem:modifiedhyper}
Fix $p\in (-1, 1)$.
Fix $d\in\N$ and $f,g: \F_2^{d}\to\F_2$. Then,
\[ \Pr_{a\sim\F_2^{d},b\sim \T_p(a)}[f(a) = g(b)=1] \le (\mu(g)\mu(f))^{1/(1+|p|)}. \] 
\end{lemma}
\begin{proof}
We can express the probability in the lemma statement as an inner product:
$\ang{f, g\circ \T_{p}}.$
Using H\"older's inequality and hypercontractivity we have
\begin{align*}
\ang{f, g\circ \T_{p}} \le \norm{f}_{1+|p|}\norm{g\circ \T_{p}}_{1+|p|} \le
\norm{f}_{1+|p|} \norm{g}_{1+|p|} \le (\mu(f)\mu(g))^{1/(1+|p|)}.
\end{align*}
\end{proof}

Now we are ready to establish the dichotomy theorem.
\begin{theorem}\label{thm:dichotomy}
Fix $p\in (-1,1)$. There exists constant $c_p$ such that the following is
true for any $d$ and functions $f,g,h,k:\F_2^{d}\to\F_2$.
Suppose $k$ has $\dist(k, \mathsf{affine})  < c_p$.
Then, the $p$-Biased $4$-function Diamond test rejects $(f,g,h,k)$ with probability at
least $\dist(k,\mathsf{affine})/2$.
\end{theorem}
\begin{proof}
Let $\chi$ be the closest affine function to $k$. Note that
\[ \chi(a)+\chi(b)=\chi(\phi_x(a,b))+\chi(\phi_x(b,a)). \] 
Thus, our goal is equivalent to showing that
\[ \Pr_{(a,x,b)\sim\DP}[(\chi+f)(a)+(\chi+g)(\phi_x(a,b))+(\chi+h)(\phi_x(b,a))\neq
(\chi+k)(b)]\ge \dist(k,\mathsf{affine})/2. \] 
Thus, it suffices to consider the case that the closest affine function to $k$
is the zero function. We assume this for the remainder of the proof. Then,
$\dist(k,\mathsf{affine})=\mu(k)$.
We are already done unless
\begin{equation}
  \label{eq:eatzero}
\Pr_{(a,x,b)\sim\DP}[f(a)+g(\phi_x(a,b))+h(\phi_x(b,a))=1]\le 2\mu(k).
\end{equation}
Thus, we may assume that \cref{eq:eatzero} is true.
Now, by \cref{lem:fghconst} we have that $f,g,h$ are $6\mu(k)$-close to
constants.
Without loss of generality we may assume $g,h$ are both closer to $0$ than to
$1$; otherwise we can add $1$ to both $g,h$, which does not affect the sum
$g(\phi_x(a,b))+h(\phi_x(b,a))$.
If $f$ were closer to $1$ than to $0$ then we would have 
\[ \Pr_{(a,x,b)\sim\DP}[f(a)=1,g(\phi_x(a,b))=h(\phi_x(b,a))=0]\ge 1-18\mu(k) > 2\mu(k), \] 
with the final inequality holding by our assumption that $\mu(k)<c_p$; but this
would contradict \cref{eq:eatzero}, so it cannot happen.
Thus, $f,g,h$ are all $6\mu(k)$-close to $0$.
% Let $$X = \setof{x}{f(x)=1\lor g(x)=1\lor h(x)=1\lor k(x)=1}.$$
% We have that $\mu(X)\le 19\mu(k)$.

Now, we return to analyzing the probability that the 4-function Diamond test
rejects $(f,g,h,k)$. This probability is at least
\[ \Pr_{(a,x,b)\sim\DP}[k(b)=1 \land f(a)=g(\phi_x(a,b))=h(\phi_x(b,a))=0]. \] 
We can lower bound this probability by 
\[ \mu(k)-\Pr_{a\sim\F_2^{d},b\sim\T_p(a)}[k(b)=f(a)=1]-\Pr_{(a,x,b)\sim\DP}[k(b)=g(\phi_x(a,b))=1]-\Pr_{(a,x,b)\sim\DP}[k(b)=h(\phi_x(b,a))=1]. \] 
Note that if $a\sim \F_2^{d},b\sim\T_p(a)$ then $\phi_x(a,b)$ is distributed as
 $\T_{(1+p)/2}(a)$
Simplifying we obtain:
\begin{equation}
  \label{eq:getreadyforhyper}
\mu(k)-\Pr_{a\sim\F_2^{d},b\sim\T_p(a)}[k(b)=f(a)=1] -
\Pr_{a\sim\F_2^{d},b\sim\T_{(1+p)/2}(a)}[k(b)=g(a)=1] - \Pr_{a\sim\F_2^{d},b\sim\T_{(1+p)/2}(a)}[k(b)=h(a)=1].
\end{equation}
Now, by \cref{lem:modifiedhyper} we can lower bound \cref{eq:getreadyforhyper} by
\begin{equation}
  \label{eq:onemore}
\mu(k)- (\mu(k)\mu(f))^{1/(1+|p|)} - (\mu(k)\mu(g))^{1/(1+(1+p)/2)} -
(\mu(k)\mu(h))^{1/(1+(1+p)/2)}.
\end{equation}
Recalling our bounds on $\mu(f),\mu(g),\mu(h)$ we can lower bound \cref{eq:onemore} by
\begin{equation}
  \label{eq:almostthere}
\mu(k)[1- 6\mu(k)^{2/(1+|p|)-1} - 12\mu(k)^{4/(p+3)-1}].
\end{equation}
Observe that the exponents on $\mu(k)$ in \cref{eq:almostthere} are bounded
above $1$ for all $p\in (-1,1)$. Thus, there is some constant $c_p$ (dependent
only on $p$ ) such that if $\mu(k)\le c_p$ then the rejection probability in
\cref{eq:almostthere} is at least $\mu(k)/2$, as desired.
\end{proof}

\subsubsection{Soundness of the $p$-biased Diamond Test}
Equipped with \cref{thm:dichotomy} we can now give the inductive analysis of the Diamond test's soundness. Ultimately we would like to show that if the 4-function Diamond test rejects $(f,g,h,k)$ with probability exactly $\eps$, then $f,g,h,k$ are all $O(\eps)$-close to affine.
So far, we have shown that if $(f,g,k,h)$ is rejected by the $4$-function
Diamond test with probability $\eps$, then $f,g,k,h$ are each \emph{either}
$c_p$-far from affine, or $2\eps$-close to affine.
We now rule out the possibility that $f$ is $c_p$-far from affine, but that the
test rejects with arbitrarily small probability.
\begin{theorem}\label{thm:induct}
Fix $p\in (-1,1)$. Let $c_p$ be the constant from \cref{thm:dichotomy}.
There is a constant $\delta_p$ such that the following holds.
Fix $d\in \N$, and functions $f,g,h,k: \F_2^{d}\to \F_2$. Suppose $f$ is
$c_p$-far from affine. Then, the $p$-Biased 4-function Diamond test rejects $(f,g,h,k)$
with probability at least $\delta_p$.
\end{theorem}

Towards the proof of \cref{thm:induct}, we will require the following Lemma from \cite{optimalreedmuller}.

\begin{lemma}[Lemma 12 of \cite{optimalreedmuller}]\label{fact:nocloserestrictions}
There exists a constant $M_p\in\N$ (dependent on $p$, but independent of $d$) such
that the following holds.
If $f:\F_2^{d}\to\F_2$ has $M_p$ many $1$-variable restrictions $f_{i,\sigma}$
which are $c_p/2$-close to affine, then $f$ is $c_p$-close to affine.
\end{lemma}
In \cite{optimalreedmuller}, the above lemma is actually bounds the number of hyperplanes on which $f$ can be close to affine, but we note that $1$-variable restrictions are also hyperplanes, and so the lemma stated above is holds as well. We state it as such as it better suits our application.

\begin{proof}[Proof of \cref{thm:induct}]
Given a function $f:\F_2^{d}\to \F_2$, coordinate $i\in [d]$, and value
$\sigma\in \F_2$, define the 1-variable restriction $f_{i,\sigma}:\F_2^{d-1}\to \F_2$ to be $f\mid_{x_i=\sigma}$.

Let $M_p$ denote the constant from \cref{fact:nocloserestrictions}.
Define $\delta_p=\min(c_p/2, (p/8)^{M_p})$.

We will prove the theorem by induction on the dimension $d$.
Our base case is $d\le M_p$.
If $d\le M_p$ then by \cref{lem:basecase} the 4-function Diamond test
rejects $(f,g,h,k)$ with non-zero probability since $f$ is not affine.
But, the smallest non-zero probability that the test could possibly reject with
is $(p/8)^d\ge (p/8)^{M_p}\ge \delta_p$.

Now, fix $d> M_p$, and assume the theorem for functions on $\F_2^{d-1}$.
Because $f$ is $c_p$-far from affine, \cref{fact:nocloserestrictions} implies
that there at most $M_p$ many 1-variable restrictions of $f$ which are
$c_p/2$-close to affine.
Thus, there is some $i\in [d]$ such the restrictions $f_{i,0}$ and $f_{i,1}$ are
both $c_p/2$-far from affine.

To analyze the probability that the 4-function Diamond test rejects $(f,g,h,k)$,
we consider a partition of the probability space into $8$ disjoint events. 
The events are the value in $\F_2^{3}$ that our sampled $(a_i,b_i,x_i)$ takes.
Now, consider the probability that the 4-function Diamond test rejects
$(f,g,h,k)$, conditional on $(a_i,b_i,x_i)=(\alpha,\beta,\xi)$ for some $\alpha,\beta,\xi$.
Conditional on this event, we will sample $a,b,x\in \F_2^{d-1}$ and check:
\[ f_{i,\alpha}(a)+g_{i,\phi_\xi(\alpha,\beta)}(\phi_x(a,b)) =
h_{i,\phi_\xi(\beta,\alpha)}(\phi_x(b,a))+k_{i,\beta}(b). \] 
This is precisely a 4-function Diamond test on $(d-1)$-dimensional functions.
Now we consider two cases.\\
\textbf{Case 1: $f_{i,\alpha}$ is $c_p$-far from affine}. \\
Then by the inductive hypothesis this $(d-1)$-dimension test will reject with
probability at least $\delta_p$.\\
\textbf{Case 2:} $\dist(f_{i,\alpha}, \mathsf{affine})\in [c_p/2, c_p]$.\\
Then, by \cref{thm:dichotomy} this $(d-1)$-dimensional diamond test rejects with
probability at least $c_p/2\ge \delta_p$.

We have seen that in all cases, the lower dimensional 4-function Diamond tests
reject with probability at least $\delta_p$.
Thus, the actual 4-function Diamond test rejects with probability $\delta_p$ as well.
\end{proof}

Combining \cref{thm:dichotomy} and \cref{thm:induct} we have get the following corollary.
\begin{corollary}\label{cor:4fun}
Fix $p\in (-1,1)$.
If $(f,g,h,k)$ passes the $p$-Biased 4-function Diamond test with probability
$1-\eps$, then $f,g,h,k$ are each $O_p(\eps)$-close to affine. 
\end{corollary}
\begin{proof}
    This result follows immediately from  \cref{thm:dichotomy} and \cref{thm:induct}.
\end{proof}
% \todo{In fact, fgjk should all be close to the same affine function modulo pushing +1's around. But Im not going to write this down right now.}
We can now conclude the proof of \cref{cor:1fun} and establish soundness for the $p$-biased Diamond test.

\begin{proof}[Proof of \cref{cor:1fun}]
    The result follows from \cref{cor:4fun} by setting $f = g = h = k$.
\end{proof}
% In fact, in the 4-function setting, we can give a slightly stronger conclusion:
% \begin{corollary}
% Fix $p\in (-1,1)$.
% Suppose $(f,g,h,k)$ passes the $p$-Biased 4-function Diamond test with probability $1-\eps$.
% Then, there is a linear function $L$ such that $f,g,h,k$ are all $O_p(\eps)$-close to either $L$ or $L+1$.
% \end{corollary}
% \begin{proof}
%  Fix such $f,g,h,k$.
%  By a union bound and \cref{fact:fliperoo} (just as in \cref{lem:4basecase}) we have:
%  there exists constants $\alpha,\beta$ such that $k$ is $2\eps$-close to $f+\alpha$, and $h$ is $2\eps$-close to $g+\beta$.
% By \cref{cor:4fun} there exist affine functions $F,G$ such that $f$ is
%  $O_p(\eps)$-close to $F$ and $g$ is $O_p(\eps)$-close to $G$.
% Then by a union bound:
% $$\Pr_{a,x\sim\F_2^{d},b\sim\T_p(a)}[F(a)+F(b)=G(\phi_x(a,b))+G(\phi_x(b,a))+\alpha+\beta]>1-O_p(\eps).$$
% Now, observe that 
% $$G(\phi_x(a,b))+G(\phi_x(b,a)) = G(a)+G(b).$$
% Thus we have
% $$\Pr_{a\sim\F_2^{d},b\sim\T_p(a)}[F(a+b)=G(a+b)+\alpha+\beta]>1-O(\eps).$$
% Thus, $f,g,h,k$ are all $O_p(\eps)$-close to either $F$ or $F+1$.
% \end{proof}



==> semi-old-stuff/simple-square-cube.tex <==
Define $S_x(a,b)$ to be the vector obtained by taking $a_i$ whenever $x_i = 0$
and $b_i$ whenever $x_i = 1$. 
Define $\Delta(a,b) \subseteq [d]$ to be the set of indices where $a,b$ differ. 
In the \defn{Linear on Subcube} test, we fix a random subcube $C_{a,b} =
\setof{x}{x_i\in \set{a_i,b_i} \forall i}$, and then run a linearity test (e.g.,
BLR \cite{BLR}) on the restricted function $f(a)+f(S_x(a,b))$.
This is the same as \cite{di19}'s Square in Cube test, which can be seen by re-writing their test as follows:
$$ (f(a)+f(S_x(a,b))) + (f(a)+f(S_y(a,b))) = f(a)+f(S_{x+y}(a,b)). $$

\begin{theorem}\label{thm:subcube}
Fix $n\in \N, d\in \N$. Suppose $f:[n]^d\to \F_2$ passes the Linear on Subcube
Test. Then $f$ is $C\eps$-close to a direct sum, for some $C$ independent of
$d,n$.
\end{theorem}
\begin{proof}
Let $\eps_{ab}$ be the probability that the $f(S_x(a,b))+f(a)$ fails the
linearity test.  Suppose $f$ passes the Linear on Subcube Test with probability
$1-\eps$. Then $\E_{ab}[\eps_{ab}] = \E_a[\eps_a] = \eps$.
Because $f(a)+f(S_x(a,b))$ passes the linearity test with probability
$1-\eps_{ab}$, there is a character $I_{ab}\subseteq \Delta(a,b)$ such that
$$
\Pr_x[f(a)+f(S_x(a,b))=\chi_{I_{ab}}(x)]>1-O(\eps_{ab}).
$$
Let $F_a(b)\in \mathbb{F}_2^{d}$ be the indicator vector for $I_{ab}\subseteq [d]$. For $v\in \F_2^d$, define $\chi_{v}(x) = \sum x_iv_i$.

\begin{lemma}\label{lem:fabdirectprod}
$F_a(b)$ is close to a direct product $(g_{1}(a,b_1),\dots,g_d(a,b_d))$
\end{lemma}

\begin{proof}
Define distribution $b'\sim D_{b}, b'\in [n]^d$ as follows: 
\begin{quote}
Sample $b'$ uniformly randomly, conditional on having $b_i'= b_i$ hold for exactly $3d/4$ of $i\in [d]$. 
\end{quote}
Define distribution $x\sim X_{bb'},x\in \mathbb{F}_2^d$ as follows:
\begin{quote}
$x_i=0$ for all $i\in \Delta(b,b')$,
and, if $b_i=b_i'$ then $x_i=1$ with probability $2/3$ and $0$ else.
\end{quote}
Observe: For any $x_{0}\in \mathbb{F}_2^d$, $\Pr_{b,b'\sim D_{b},x\sim X_{bb'}}[x=x_{0}]=1/2^d$. 
That is, $x$ is uniformly distributed, and pairwise independent of $b,b'$, although of course the triple $(x,b,b')$ is not uniformly random on $\F_2^d \times [n]^d\times [n]^d$. 
By construction, $S_x(a,b) = S_x(a,b')$ (whenever $b_i,b_i'$ differ, we choose $a_i$).
Then, by a union bound (and averaging away $b$ in our earlier expression) we have that 
$$
\Pr_{b,b'\sim D_{b},x\sim X_{bb'}} [\chi_{F_a(b)}(x) =f(a)+f(S_x(a,b)) = f(a)+f(S_x(a,b')) = \chi_{F_a(b')}(x)] > 1-2\eps_{a}.
$$
Let 
$$
\delta_{abb'} =  \Pr_{x\sim X_{bb'}} [\chi_{F_a(b)\oplus F_a(b')}(x) \neq 0].
$$
Let $\overline{\Delta}(b,b')$ denote the set of indices $i$ where $b_i=b_i'$. For vector $x\in \mathbb{F}_2^d$, and set $S\subseteq [d]$, let $x\mid_S$ denote the restriction of $x$ to coordinates $S$. Then,

\begin{claim}
If $\delta_{abb'}<1/3$ then $F_a(b)\mid_{\overline{\Delta}(b,b')}= F_a(b')\mid_{\overline{\Delta}(b,b')}$.
\end{claim}
\begin{proof}
Assume for sake of contradiction that there exists  $i\in \Delta(F_a(b), F_a(b')) \cap \overline{\Delta}(b,b')$.\\
Sampling $x\sim X_{bb'}$ we have a $1/3$ chance of $x_i$ being $0$ and a $2/3$ chance of $x_i$ being $1$, independent of the values of $x_j$ for $j\neq i$.\\
But then $\chi_{F_a(b)\oplus F_a(b')}(x)$ doesn't take on any value in $\mathbb{F}_2$ with probability greater than $2/3$, contradicting $\delta_{abb'}<1/3$.\\
Thus, $\Delta(F_a(b), F_a(b')) \cap \overline{\Delta}(b,b') = \varnothing$.
\end{proof}

Now, by Markov's Inequality we have that 
$$
\Pr_{b,b'\sim D_{b}}[\delta_{abb'}>1/3] \le 3\mathbb{E}_{b,b'}[\delta_{abb'}] < 6\eps_a.
$$
From this we conclude
$$
\Pr_{b,b'\sim D_{b}} [F_a(b)\mid_{\overline{\Delta}(b,b')}= F_a(b')\mid_{\overline{\Delta}(b,b')}] > 1-6\eps_a.
$$
By the direct product theorem we conclude that $F_a(b)$ is $O(\eps_a)$-close to a direct product $(g_1(a,b_1),\dots,g_d(a,b_d))$. 
Combining these facts we have:
$$ 
\Pr_{x,b} \left[ f(a)+f(S_x(a,b)) = \sum_i g_i(a,b_i)x_i \right] > 1-O(\eps_a). 
$$
This concludes the proof of \cref{lem:fabdirectprod}.
\end{proof}

Now we prove the theorem.
Observe that $S_{x}(a,b)=S_{\bar{x}}(b,a)$. Thus, by \cref{lem:fabdirectprod} and a union bound,
$$
\Pr_{a,b,x} \left[ \sum_{i}g_{i}(a,b_{i})x_{i}= f(a)+f(S_x(a,b))=f(b)+f(S_{\bar{x}}(b,a))=\sum_{i}g_{i}(b,a_{i})\overline{x_{i}} \right]>1-O(\eps).
$$
Define 
$$
\lambda_{ab}=\Pr_x\left[ \sum_i (g_i(a,b_i)+g_i(b,a_i))x_i \neq \sum_i g_i(b,a_i) + f(a)+f(b) \right].
$$
Clearly, if $\lambda_{ab}<1/2$  then we must have 
$$
\sum_i g_i(b,a_i)=f(a)+f(b).
$$
By Markov's inequality:
$$
\Pr_{a,b}[\lambda_{ab}>1/2]< 2\mathbb{E}_{a,b}[\lambda_{ab}]< O(\eps).
$$
Thus, we have:
$$
\Pr_{a,b}\left[ f(a)=f(b)+\sum_i g_i(b,a_i)  \right] > 1-O(\eps).
$$
Then, by the probabilistic method there exists $\beta$ such that 
$$
\Pr_a\left[ f(a)=f(\beta)+\sum_i g_i(\beta,a_i) \right]>1-O(\eps).
$$
That is, $f$ is $O(\eps)$-close to the direct sum $a\mapsto f(\beta)+\sum_i g_i(\beta,a_i)$.

\end{proof}    

==> semi-old-stuff/smallepsilon.tex <==
\subsection{A Close-Far Dichotomy for the Diamond Test}
The first step in our analysis will be to establish the following dichotomy for
functions passing the diamond test with good probability:
\begin{lemma}\label{lem:dichotomy}
Fix $\rho\in (-1,1), d\in \N, f:\F_2^{d}\to \F_2$, and let $\eps$ be the
probability that the $\rho$-Diamond test rejects $f$.
Then, either $f$ is $4^{(3+\rho)/(\rho-1)}$-far from affine, or $f$ is $2\eps$-close to affine.
\end{lemma}
\begin{proof}
Fix $\rho,d,f,\eps$ as in the lemma statement.  We may assume $\eps\le 1/4$ or
else we are already done. Let $\chi_0$ be the closest affine function to $f$. 
Because $\chi_0$ passes the Diamond test with probability $1$ (as shown in \cref{lem:rhobasecase}), we have that $f+\chi_0$ passes the Diamond test with probability exactly $1-\eps$ just like $f$.
We assume $\dist(f, \mathsf{affine}) > 2\eps$, and aim to show $\dist(f, \mathsf{affine}) \ge 4^{(3+\rho)/(\rho-1)}$.
Let $X$ denote the support of $f+\chi_0$. Clearly $x\mapsto 0$  is the closest affine function to $f+\chi_{0}$. Thus we have 
$$\mu(X)\coloneq \Pr_{a\sim \F_2^d}[a\in X] = \dist(f+\chi_0, \mathsf{affine}) = \dist(f, \mathsf{affine}) > 2\eps,$$
and our goal is to show that $\mu(X)\ge 1/4^{1+2/(1+p)}$.

In order for the Diamond test to reject $f+\chi_{S_0}$ with probability $\eps$ we must have:
\begin{equation}
\Pr_{a,x\sim \F_2^d,b\sim \T_\rho(a)}[a\in X \land \set{b,\phi_x(a,b),\phi_x(b,a)}\subseteq \overline{X}] \le \eps/2.
\end{equation}
Therefore, 
$$ \mu(X)\cdot \Pr_{a\sim X, b\sim \T_\rho(x), x\sim\F_2^d}\left[\set{b,\phi_x(a,b),\phi_x(b,a)}\subseteq\overline{X}\right] \le \eps/2. $$ 
Because $\mu(X)>2\eps$, we have
$$ \Pr_{a\sim X, b\sim \T_\rho(x), x\sim\F_2^d}\left[\set{b,\phi_x(a,b),\phi_x(b,a)}\subseteq\overline{X}\right] < 1/4. $$ 
Thus, 
$$ \Pr_{a\sim X, b\sim \T_\rho(x), x\sim\F_2^d}\left[b\in X \lor \phi_x(a,b)\in X \lor \phi_x(b,a)\in X \right] > 3/4. $$ 
By the union bound
$$ 3/4 < \Pr_{a\sim X, b\sim \T_\rho(x), x\sim\F_2^d}[b\in X] +  2\Pr_{a\sim X, b\sim \T_\rho(x), x\sim\F_2^d}[\phi_x(a,b)\in X]. $$ 
The distribution of $\phi_x(a,b)$ induced by $b\sim\T_\rho(x),x\sim\F_2^d$ is $\T_{(1+\rho)/2}(a)$. Thus,
\begin{equation}\label{eq:almosthyper}
3/4 < \Pr_{a\sim X, b\sim \T_\rho(x)}[b\in X] +  2\Pr_{a\sim X, b\sim \T_{(1+\rho)/2}(x)}[b\in X].
\end{equation}
% Hence, 
% $$ 1/8+\eps > 1-\Pr_{a\in 1[f], b, x}\left[a_xb\in1[f] \bigvee b_xa \in 1[f]\right] \ge 1-2\Pr_{a\in 1[f],b,x}\left[a_xb\in 1[f]\right]. $$ 
% Therefore, 
% $$
% \Pr_{a\in 1[f],b,x}\left[a_xb\in 1[f]\right] \ge 1/2 - (1/16+\eps/2)\ge 1/4.
% $$
% Now we can phrase this in terms of the \defn{noise operator}. Specifically,
% $\mathsf{T}_{1/2}(x)$ is a distribution on $\F_2^d$ obtained as follows: set the
% $i$-th value to $x_i$ with probability $3/4$ and $x_i+1$ with probability $1/4$.
% It is clear that the distribution of $a_xb$ for fixed $a$ and uniform $b,x$ is
% precisely $\mathsf{T}_{1/2}(a)$.
% Thus, we have shown:
% $$\Pr_{a\in 1[f], a'\sim \mathsf{T}_{1/2}(a)}\left[a'\in 1[f]\right] \ge 1/4.$$
A classic fact of Fourier analysis (\cite{hyper1},\cite{hyper2}) is that the
noisy hypercube is a \defn{small set expander}. Specifically we have (\cite{od21}):
\begin{fact}[Small Set Expansion of the Noisy Hypercube]
$$ \Pr_{a\sim X, b\sim \mathsf{T}_{p}(a)}[b\in X] \le \mu(X)^{(1-p)/(1+p)}. $$
\end{fact}
Applying this in \cref{eq:almosthyper} gives:
$$3/4 < \mu(X)^{(1-\rho)/(1+\rho)}+2\mu(X)^{(1-\rho)/(3+\rho)} \le 3\mu(X)^{(1-\rho)/(3+\rho)}.$$
Thus, 
$$\mu(X) > 1/4^{(3+\rho)/(1-\rho)},$$
as claimed.

\end{proof}


==> semi-old-stuff/strong_diamond.tex <==
\subsection{An Inductive Analysis of the Diamond Test}

\begin{theorem}
Fix $f:\F_2^{d}\to \F_2$, and let $\eps$ be the probability that the diamond test
rejects $f$.
Then, $f$ is $1000\eps$-close to affine.
\todo{could be nice to get a better constant here.}
\end{theorem}
\begin{proof}
First, we note that the theorem is vacuously true for $\eps\ge .00001$, so we will
assume $\eps < .00001$.

\todo{EDIT: we need to assume $d>1000$ or something.
This is fine. but just say it.}

We prove the theorem by induction on $d$. 
The base case $d=1$ is trivially true; all one dimensional functions are affine.
Now, suppose the theorem is true for dimension $d-1$.
Fix $f:\F_2^{d} \to \F_2$ which passes the diamond test with probability
$1-\eps>.9999$.

\todo{rename b to sigma}
For each $i\in [d], b\in \F_2$  define function $f_{i,b}$ to be $f$, except with
the $i$-th input bit fixed to value $b$.
We claim that $f_{i,b}$ passes the diamond test with probability at least
$1-4\eps$. Indeed, there is a $1/4$ chance that our diamond test on $f$ amounts
to a diamond test on $f_{i,b}$.
By the inductive hypothesis, we now infer that each $f_{i,b}$ is
$1000\eps$-close to affine.

We claim that this will imply that $f$ is close to affine.

Suppose we run (affine) BLR on $f$.
For each $i,b$ let $P_{i,b}$ be the event that the BLR selects all the
coordinates $z,x+z,y+z,x+y+z$ to be bit  $b$.
Then $\Pr[P_{i,b}] = 1/4,$
and $P_{i,b} \perp P_{i',b'}$ if $(i,b)\neq (i',b')$.
Let $\pi$ be the event that the BLR test on $f$ passes
Observe that $\Pr[\pi \mid P_{i,b}] > 1-1000\eps$ in light of our earlier
observation.

Define event $L_{i,b} = P_{i,b} \land \overline{\pi}$. 
In light of the above observation we have:
\[ \Pr [\bigvee_{i=1}^{1000}L_{i,0}] \le 1000000 \eps. \] 

Now observe:
\[ \Pr[\pi] \ge \Pr[\bigvee_{i=1}^{1000}P_{i,0} \land \neg
\bigvee_{i=1}^{1000}L_{i,0} ]. \] 
Then, 
\[ \Pr[\overline{\pi}] \le (3/4)^{1000} + 100000\eps.  \] 

Remember we assumed $\eps$ is small so we win.

In summary, we have shown that $f$ is $100000\eps$-close to affine.
But, recall that we had a dichotomy: 
either $f$ is really far, or really close. 
So we boost and win.
Induction completed. 

\todo{RIP this is false.}

\end{proof}



==> simple_restrictions.tex <==
\begin{proof}
We take $N$ to be large enough so that $(1-1/n)^{N/n} < c/2$ and so that
$N> 10n^2$.

Let $Y \subseteq [d]$ be the set of variables $i$ such that $f$ has a
$1$-variable restriction at coordinate $i$ which is $\eps$-close to a direct
sum. By the pigeonhole principle $f$ has at least $N/n$ $1$-variable
restrictions of distinct coordinates. Without loss of generality, we assume that
for each $i\in Y$, the restriction $f\mid_{x_i = 1}$ is  $\eps$-close to a
direct sum. Then, there are direct sums $L^{(i)}:[n]^{d-1}\to \F_2$ for each
$i\in Y$ such that \[ \Pr_x[f(x) = L^{(i)}(x_{-i}) \mid x_i = 1] \ge 1-\eps. \] 

Now we observe an agreement between the $L^{(i)}$'s.
For any $i,j\in Y$ we must have
\begin{equation}
  \label{3eq:L_agree}
\Pr_x[L^{(i)}(x_{-i}) = f(x)=L^{(j)}(x_{-j}) \mid x_i = x_j = 1] \ge 1-2n\eps.
\end{equation}
Re-index the variables so that the variables in $Y$ are $x_1,x_2,\ldots, x_{|Y|}$.
Now, recall that the minimum distance for direct sums is $1/n$; thus, using
$\eps<\frac{1}{10n^2}$ in \cref{3eq:L_agree} we have that for all $i,j\in Y$, 
\[L^{(i)}\mid_{x_j=1} = L^{(j)}\mid_{x_i=1}.\]
Now, define $L:[n]^{d}\to \F_2$ as follows:
\[ L(x) = L^{(2)}_1(x_1) + \sum_{i=2}^d L^{(1)}_i(x_i), \] 
where we have defined $L^{(j)}(x_{-1}) = \sum_{i\neq j} L^{(j)}_i(x_i)$.
For any $i \in Y$ we have
\[ L\mid_{x_i=1} = L^{(i)}. \] 
Thus, for any $i\in Y$ we have
\[ \Pr_x[f(x) = L(x) \mid x_i = 1] \ge 1-\eps. \] 
Now we have
\begin{align*}
\Pr_x[f(x)=L(x)] &\ge \Pr_x\left[ \bigwedge_{i\in Y} \overline{[x_i=1 \land f(x)\neq L(x)]} \land \bigvee_{i\in Y}[x_i=1] \right] \\
&\ge \Pr_x\left[ \bigvee_{i\in Y}[x_i=1] \right] - \Pr_x \left[ \bigvee_{i\in Y}[x_i=1 \land f(x)\neq L(x)] \right] \\
&\ge \Pr_x\left[ \bigvee_{i\in Y}[x_i=1] \right] - |Y| \frac{\eps}{n} \\
&\ge 1-(1-1/n)^{|Y|} - |Y| \frac{\eps}{n} \\
&\ge 1-c/2 - |Y| \frac{\eps}{n} \\
\ge 1-c.
\end{align*}
That is, $f$ is $c$-close to direct sum $L$.
\end{proof}


==> weak-diamond.tex <==
\subsection{A Weak Analysis of the Diamond Test}

In this section we show that the diamond test is at least somewhat good at rejecting functions which are far from affine: if $f$ is $\eps$ far from affine, the Diamond test rejects with probability $\Omega(\eps/d^{1.1})$.
The dependence on $d$ is undesirable, and in future sections we will discuss attempts at achieving stronger quantitative results.

\todo{more description text here}

\begin{lemma}\label{lem:bday}
    Suppose $X\subset \F_2^d$  has $|X|\ge .99 |\F_2^d|$, and let $d$ be at
    least a sufficiently large constant.
    Then, there exists a subset $B\subset X$, with $|B|= \ceil{1.02\log_2 d}$, 
    such that for any $i\in [d]$ $B$ contains both a vector $x$ with $x_i = 1$
    and a vector $x'$ with $x_i'=0$.
\end{lemma}
\begin{proof}
By the probabilistic method it is sufficient to demonstrate that a randomly chosen $B\subset X$ has the desired property with non-zero probability. 
Fix some coordinate $i\in [d]$.
The probability that $B$ only contains vectors of a single parity at coordinate $i$ is at most
$$2(100/198)^{\ceil{1.02\log_2 d}}< 1/(2d).$$
By a union bound the probability that there is any coordinate where $B$ lacks vectors of both parities at the coordinate is at most $1/2$.
\end{proof}

\begin{lemma}\label{lem:diamond}
There exist $b,c$ such that 
$$
\Pr_{a,x}\left[f(a)=f(a_xb)f(c_xa)f(c_xb)\right]>1-2\eps.
$$
\end{lemma}
\begin{proof}
We perform the following two tests:
$$
f((a_xd)_xb)f(b_x(a_xd)) = f(a_xd)f(b)
$$
$$
f(b_x(c_xd))f((c_xd)_xb) = f(c_xd)f(b).
$$
It may be more clear to think of these like this:
$$
f(a_xb)f(b_xd) = f(a_xd)f(b)
$$
$$
f(b_xd)f(c_xb) = f(c_xd)f(b).
$$
If $a,b,c,d,x$ are sampled uniformly randomly then these are both uniformly random tests, although they are correlated. 
By a union bound, the tests simultaneously pass with probability $1-2\eps$.
Thus, we have 
$$\Pr_{a,b,c,d,x}\left[f(a_xb)f(a_xd)=f(c_xd)f(c_xb)\right]>1-2\eps.$$
Renaming variables again we get:
$$
\Pr_{a,c,d,x}\left[f(a) = f(a_xd)f(c_xd)f(c_xa)\right]>1-2\eps.
$$
By the probabilistic method we can choose $c,d$ such that 
$$\Pr_{a,x}\left[f(a) = f(a_xd)f(c_xd)f(c_xa)\right]>1-2\eps.$$
\end{proof}

\begin{lemma}
\label{lem:refine}
Suppose there is a partition $I=(I_1,\ldots, I_k)$  of $[d]$ and there are functions $g_1,\ldots, g_k$ with $g_i: \F_2^{I_i}\to \pm 1$, and there is $\xi$ such that:
$$
\Pr_a \left[f(a) = \prod_i g_i(a_{I_i})\right]>1-\xi.
$$
Suppose further that there exists a partition $J_0\sqcup J_1=[d]$ and functions $h_0:\F_2^{J_0}\to \pm 1,h_1:[2]^{J_1}\to\F_2$ and $\eps$  such that 
$$\Pr_a \left[f(a) = \prod_j h_j(a_{J_j})\right]>1-\eps.$$
Then there exist functions $\ell_{i,j}:[2]^{I_i\cap J_j}\to \F_2$ such that 
$$\Pr_a\left[  f(a) = \prod_{i,j}\ell_{i,j}(x_{I_i\cap J_j}) \right] > 1-2(\eps+\xi)-\eps.$$
\end{lemma}
\begin{proof}
By a union bound, with probability $\eps+\xi$ over choice of $a$ we get:
$$
\prod_i g_i(a_{I_i}) = \prod_j h_j(a_{J_j}).
$$
For each $j$, by the probabilistic method, there exists $a_{\overline{J_j}}$ such that 
$$\Pr_{a_{J_j}} \left[h_j(a_{J_j}) = h_{j+1}(a_{\overline{J_{j}}}) 
\prod_i g_i(a_{I_i})
\right] > 1-(\eps+\xi).$$
We can interpret this as the existence of the $\ell_{i,j}:[2]^{I_i\cap J_j}\to \F_2$ described in the lemma statement.
Finally, by another union bound we have 
$$\Pr_a\left[  f(a) = \prod_{i,j}\ell_{i,j}(x_{I_i\cap J_j}) \right] > 1-2(\eps+\xi)-\eps.$$
\end{proof}

Now we combine the three lemmas to prove the following:
\begin{theorem}
    If $f:\F_2^d \to \pm 1$ passes the diamond test with probability $\eps$ then is is at least $O(d^{1.02}\eps)$ close to linear. 
\end{theorem}
\begin{proof}
Call $x$ \defn{good} if 
$$\Pr_a[f(a) = f(a_xb)f(c_xa)f(c_xb)]>1-100\eps.$$
By \cref{lem:diamond} we have:
$$\E_x[\Pr_a[f(a) \neq f(a_xb)f(c_xa)f(c_xb)]]<2\eps.$$
Thus, by Markov's Inequality, at least $99$\% of $x$ are good.
Now, by \cref{lem:bday} we can find good $x^{(1)},\ldots, x^{(\ceil{1.02\log d})}$ such that for each $i\in [d], b\in \F_2$ there is some vector $x^{(j)}$ with $x^{(j)}_i=b$.
Now we repeatedly apply \cref{lem:refine} and XXX.

\todo{finish some details}
\end{proof}
